Controller Design and Implementation of a New Quadrotor Manipulation System

The previously introduced aerial manipulation systems suffer from either limited end-effector DOF or small payload capacity. In this dissertation, a quadrotor with a 2-DOF manipulator is investigated that has a unique topology to enable the end-effector to track 6-DOF trajectory with the minimum possible number of actuators/links and hence, maximize the payload and/or mission time. The proposed system is designed, modeled, and constructed. An identification process is carried out to find the system parameters. An experimental setup is proposed with a 6-DOF state measurement and estimation scheme. The system feasibility is validated via numerical and experimental results. The inverse kinematics require a solution of complicated algebraic-differential equations. Therefore, an algorithm is developed to get an approximate solution of these equations.

==> 0_frontmatter/SUMMARY.tex <==

% Thesis Abstract -------------------------------

\begin{abstract}       

The research on aerial manipulation has been increased rapidly in recent years due to its unique features that qualify it to be utilized in vital applications and to support human in daily life activities. In the previous works, a manipulator or a gripper is attached to the bottom of a quadrotor to facilitate the interaction with the environment. However, the previous introduced systems suffer from either limited end-effector Degrees Of Freedom (DOF) or small payload capacity. The systems that use a gripper suffer from the limited allowable DOF of the end-effector. The other systems have a manipulator with either two DOF but in certain topology that disables the end-effector to track arbitrary 6-DOF trajectory, or more than two DOF that decreases greatly the possible payload carried by the system. In this dissertation,  a quadrotor with a 2-DOF manipulator is investigated that has a unique topology to enable the end-effector to track 6-DOF trajectory with minimum possible number of actuators/links and hence, maximize the payload and/or mission time. The proposed system is designed, modeled, and constructed. An identification process is carried out to find the system parameters. The currently developed quadrotor-based aerial manipulators depend on a high cost 3D motion capture system to estimate the system states which will restrict the functions of the system to be within limited space indoors. Therefore, an experimental setup is proposed with a 6-DOF state measurement and estimation scheme that can be utilized within arbitrary places indoors and it has a potential to work outdoors as well. The system feasibility is validated via numerical and experimental results. The proposed non-redundant system has complexity in its inverse kinematics that are required in order to transform task space trajectory to quadrotor/joint space trajectory. Such inverse kinematics require a solution of complicated algebraic-differential equations. The differential equations represent the higher-order nonholonomic constraints of the system. Therefore, an algorithm is developed to get an approximate solution of these equations. The accuracy of the solution is verified via numerical simulations. Moreover, the success of the inverse kinematics analysis proves the ability of the system to track arbitrary 6-DOF task space trajectories that lay within the capability of the system constraints. Furthermore, the motion control of this quadrotor manipulation system is quite challenging. The system has strong nonlinearities and fast dynamics. There are complex couplings among its variables. In addition, it is naturally unstable and very susceptible to parameters variations, external disturbances (e.g., wind), noisy measurements, and actuators' faults. Thus, a linear Disturbance Observer (DOb)-based robust control technique is utilized to address these issues. A modified DOb loop is proposed and designed to use the direct measurements from the onboard sensors in order to reduce the disturbance estimation error. For the optimization of the control signal, to save power consumption and thus to increase the mission time, as well as the consideration of the actuators' constraints, a Model Predictive Control (MPC) is used in the external loop of the DOb to achieve these objectives.  In addition to the accurate positioning of the end-effector, the manipulation tasks require estimating (applying) certain force at the end-effector as well. However, the current developed techniques have limitations because they are model-based methods, and they are based on ignoring some dynamics and/or requiring an indicator of the environment contact. Therefore, a robust sensorless force estimation and impedance control scheme is proposed to overcome these limitations based on both the robust linearization capabilities of the DOb and the Fast Tracking Recursive Least Squares (FTRLS) algorithm. The efficiency of the proposed control systems is validated via numerical results.

\end{abstract}



% ----------------------------------------------

==> 1_Introduction/Introduction.tex <==

% this file is called up by thesis.tex
% content in this file will be fed into the main document

%: ----------------------- introduction file header -----------------------
\chapter{INTRODUCTION}
\label{ch:Introduction}

%: ----------------------- paths to graphics ------------------------
% the code below specifies where the figures are stored
\ifpdf
    \graphicspath{{1_Introduction/figures/}}
\else
    \graphicspath{{1_Introduction/figures/}}
\fi

% 
%: ----------------------- introduction content -----------------------

In this chapter, the research background on the aerial manipulation systems, which induces the motivation of this research, is presented. The objectives of this research are clearly described and the outline of the thesis is
briefly introduced. 

\section{Research Background}

\subsection{Overview of the Current Developed Aerial Manipulators}

Recently, the evolvement of technology is much more concentrating on improving the standard of human living. Robots and mechatronic systems are expected to
support human activities in daily life, industry, entertainment, service, outer space and
medicine. Such activities include; inspection, maintenance, firefighting, service robot in crowded cities to deliver light stuff such as post mails or quick meals, rescue operation, surveillance, demining, performing tasks in dangerous places (e.g., Nuclear stations), or transportation in remote places (see Fig. \ref{fig:qms_apps}). 
%============================================== 
\begin{figure}[!h]
	\centering
	\begin{tabular}{cc}
			\subfloat[Search \& rescue in a disaster area \cite{weiss2012vision}]{\includegraphics[height=5.26 cm,width=0.5\columnwidth]{rescue}}&	
		\subfloat[Demining \cite{demining_ref}]{\includegraphics[width=0.5\columnwidth]{deming}}\\
		\subfloat[Accessing difficult terrains \cite{terran_ref}]{\includegraphics[width=0.5\columnwidth]{difficult_terran}}&
		\subfloat[Maintenance in nuclear station \cite{nuclear_ref}]{\includegraphics[width=0.5\columnwidth]{nuclear_station}}\\
	\end{tabular}
	\caption{Examples of tasks that need robotics especially aerial robots}
	\label{fig:qms_apps}
\end{figure}
%============================================

There are two main categories of the robotic systems; ground robots and aerial robots. However, the ground robots have constraints and limitations to move and access all types of the environments and terrains. Recently, the aerial vehicles are utilized to overcome these constraints and they offer possibilities of speed and access to regions that are otherwise inaccessible to ground robotic vehicles. There are several types of aerial vehicles (fixed wing, helicopters, single rotor, twin rotor, quadrotor, hexacopter, octocopter, $\ldots$, etc). Quadrotor system (see Fig. \ref{fig:typical_quadrotor}) is one of the Unmanned Aerial Vehicles (UAVs) which possess certain essential characteristics, such as small size and cost, Vertical Take Off and Landing (VTOL), performing slow precise movements, and impressive maneuverability, which highlight its potential for use in vital applications. Such applications include; homeland security (e.g. Border patrol and surveillance), military surveillance, service and rescue tasks, and earth sciences (to study climate change, glacier dynamics, and volcanic activity) \cite{quad_survey}. However, most research on UAVs has typically been limited to  monitoring and surveillance applications where the objectives are limited to "look" and "search" but "do not touch". Due to their superior mobility, much interest is given to utilize them for aerial manipulation. 
% =======================================
\begin{figure}
	\centering
	\includegraphics[width=0.4\columnwidth]{typical_quadrotor}
	\caption{Typical quadrotor \cite{quad_ref}}
	\label{fig:typical_quadrotor}
\end{figure}
% ===========================================
Previous research on the quadrotor-based aerial manipulation systems can be divided into three approaches. 

In the first approach, a gripper or a tool  is installed at the bottom of an UAV to transport a payload or interact with existing structures, see Fig. \ref{fig:quad_gripper}. In \cite{Aerial_Grasping, lindsey2012construction, willmann2012aerial}, a quadrotor with a gripper is used for transporting blocks and to build structures. In \cite{albers2010semi}, a force sensor is used to apply a normal force to a surface. Accordingly, not only the attitude of the payload/tool is restricted to the attitude of the UAV, but also the accessible range of the end-effector is confined due to the fixed configuration of the gripper/tool with respect to the UAV body and blades. Consequently, the resulting aerial system has 4 Degrees Of Freedom (DOF); three translational DOF and one rotational DOF (Yaw), i.e., the gripper/tool cannot posses pitch or roll rotation without moving horizontally. 


% =======================================
\begin{figure}[h]
	\centering
	\includegraphics[width=0.4\columnwidth]{quad_gripper}
	\caption{Quadrotor carrying a payload via a gripper \cite{Aerial_Grasping}}
	\label{fig:quad_gripper}
\end{figure}
% ===========================================
The second approach is to suspend a payload with cables, see Fig. \ref{fig:quad_cables}. In \cite{bisgaard2010adaptive}, an adaptive controller is presented to avoid swing excitation of a payload. In \cite{michael2011cooperative, goodarzi2015geometric, goodarzi2015dynamics}, specific attitude and position of a payload is achieved using cables connected to one or three quadrotors. However, this approach has a drawback that the movement of the payload cannot be always regulated directly because the manipulation is achieved using a cable which cannot always drive the motion of the payload as desired.  
% =======================================
\begin{figure}[h]
	\centering
	\includegraphics[width=0.4\columnwidth]{quad_cables}
	\caption{Quadrotor carrying a payload via a cable \cite{bisgaard2010adaptive}}
	\label{fig:quad_cables}
\end{figure}
% ===========================================
To overcome these limitations, a third approach is developed in which an aerial vehicle is equipped with a robotic manipulator that can actively interact with the environment. For example, in \cite{korpela2012mm}, a test bed including two 4-DOF robot arms and a crane emulating an aerial robot is proposed. By combining the mobility of the aerial vehicle with the versatility of a robotic manipulator, the utility of mobile manipulation can be maximized. When employing the robotic manipulator, the dynamics of the robotic manipulator are highly coupled with that of the aerial vehicle, which should be carefully considered in the controller design. In addition, an aerial robot needs to tolerate the reaction forces from the interactions with the object or external environment. These reaction forces may affect the stability of an aerial vehicle significantly. Very few reports exist in the literature investigate the combination of aerial vehicle with robotic manipulator. 
In \cite{thomas2013avian}, the authors propose a flying robot that can similarly swoop down and grab objects in the way that an
eagle can fish with its natural claws. Their proposed system consists of a quadrotor with a 1-DOF robotic arm, see Fig. \ref{fig:quad_eagle}. 
% =======================================
\begin{figure}[h]
	\centering
	\includegraphics[width=0.4\columnwidth]{quad_eagle}
	\caption{Swooping quadrotor with claws \cite{thomas2013avian}}
	\label{fig:quad_eagle}
\end{figure}
% ===========================================
Kinematic and dynamic models of the quadrotor combined with arbitrary multi-DOF robot arm are derived using the Euler-Lagrangian formalism in \cite{lippiello2012cartesian}. Based on that, simulation results using the Cartesian impedance control for the combined system with 3-DOF robotic arm is presented in \cite{lippiello2012exploiting}. In addition, the effects of manipulators, two 4-DOF arms, on the quadrotor are simulated based on the dynamic model which considers a quadrotor and robotic arms separately, treating the arms as the disturbance to the quadrotor control loop. In \cite{orsag2013modeling}, a quadrotor with light-weight manipulators, three 2-DOF arms, are tested, although the movement of the manipulators is not explicitly considered during the design of the PID controller (see Fig. \ref{fig:3_2-dof_quad_manp}). 
% =======================================
\begin{figure}
	\centering
	\includegraphics[width=0.4\columnwidth]{3_2-dof_quad_manp}
	\caption{Quadrotor carrying a payload via three 2-DOF arms \cite{orsag2013modeling}}
	\label{fig:3_2-dof_quad_manp}
\end{figure}
% ===========================================
In \cite{ruggieromultilayer, heredia2014control, cano2013mechanical} a manipulator with more than two links were used. However, with these systems, the final payload of the quadrotor is decreased due to the excessive manipulator weight, see Fig. \ref{fig:quad_6dof_manp}.    
% =======================================
\begin{figure}
	\centering
	\includegraphics[width=0.4\columnwidth]{quad_6dof_manp}
	\caption{Quadrotor carrying a payload via 6-DOF arm \cite{heredia2014control}}
	\label{fig:quad_6dof_manp}
\end{figure}
% ===========================================
In \cite{kim2013aerial}, an aerial manipulation using a quadrotor with a 2-DOF robotic arm is presented but with certain topology that disable the system from making arbitrary position and orientation of the end-effector as shown in Fig. \ref{fig:quad_2dof_manp}. In this system, the axes of the manipulator joints are parallel to each other and parallel to one in-plane axis of the quadrotor. Thus, the system cannot achieve orientation around the second in-plane axis of the quadrotor without moving horizontally.
% =======================================
\begin{figure}[h]
	\centering
	\includegraphics[width=0.4\columnwidth]{quad_2dof_manp}
	\caption{Quadrotor carrying a payload via 2-DOF robotic arm in with parallel joints' axes \cite{kim2013aerial}}
	\label{fig:quad_2dof_manp}
\end{figure}
% ===========================================

From the above discussion, the systems that use a gripper suffer from the limited allowable DOFs of the end-effector. The other systems have a manipulator with either two DOFs but in certain topology that disables the end-effector to track arbitrary 6-DOF trajectory, or more than two DOFs which decreases greatly the possible payload carried by the system.

In \cite{new_quad_manp, khalifa2013adaptive}, a new aerial manipulation system is proposed that consists of 2-link manipulator, with two revolute joints whose axes are perpendicular to each other and the axis of the first joint is parallel to one in-plane axis of the quadrotor, see Fig. \ref{fig:our_quad_2dof_manp}. Thus, the end-effector is able to reach arbitrary position and orientation without moving horizontally. However, the proof that this system can perform any desired trajectory in the task space has not been achieved yet due to the resulted complications in the inverse kinematics and control. This system is similar to a serial manipulator with eight joints, two of them are passive. In this research, a novel inverse kinematics analysis is presented to prove and test the robot capability to track a 6-DOF task space trajectories. Moreover, controller design is carried out that makes use of the inverse kinematics solution to track arbitrary 6-DOF task space trajectory. Also, experimental implementation of the system is carried out to check its capabilities which is not done before.
% =======================================
\begin{figure}
	\centering
	\includegraphics[width=0.4\columnwidth]{our_quad_2dof_manp}
	\caption{Quadrotor carrying a payload via 2-DOF robotic arm that has unique topology \cite{new_quad_manp}}
	\label{fig:our_quad_2dof_manp}
\end{figure}
% ===========================================

\subsection{Experimental Setup and Measurements}

One of the key issues in  the aerial manipulation system is achieving the position holding task. To do this task, the accurate measurements and estimation of the system states must be achieved. However, all the current developed systems \cite{thomas2013avian, choi2015nonlinear, ghadiok2012design, kim2013aerial, ruggiero2015multilayer, baizid2015experiments} use a positioning scheme that depends on a high cost 3D Motion Capture System (e.g., VICON system) which will restrict the functions of the aerial manipulation to be within limited space indoors. However, most real applications require to do tasks in arbitrary places indoors and/or outdoors. Therefore, in this work, a proposed solution to this issue is presented and tested that is based on using onboard sensors. The experiments are carried out for point-to-point control using position holding strategy in teleoperation framework rather than trajectory tracking control. Autonomous trajectory tracking control needs high accurate sensing system which is not available.   

\subsection{Control System}

The control of the quadrotor manipulation system is quite challenging because it is naturally unstable, and has strong nonlinearities. In addition, it is very susceptible to parameters variations due to adding/releasing the payload and the actuators' losses. Moreover, it is subjected to external disturbances like wind. Furthermore, its measurements are very noisy due to the thrusters that rotate at very high speed. Also, it has fast dynamics. Therefore, there is a need to design and implement an efficient and low computational cost robust control technique to address these issues.

Furthermore, the actuators (thrusters and manipulator motors) have constraints, which may degrade the performance if it is not considered during controller design. Moreover, it is had to apply an optimal control effort to reduce the required power of the thrusters such that one can save power and thus increase the mission time. Therefore, a Model Predictive Control (MPC) based control technique is proposed to address this issue.


In the motion control of the aerial manipulator, achievement of the compliance control is very important because the compliance control makes possible to perform flexible motion of the manipulator according to a desired impedance. In addition, for the teleoperation purpose, the users may need to sense the force applied at the end-effector. This is very critical demand in applications such as demining and maintenance. Therefore, one have to design a sensorless force estimation to avoid the complicated design resulted from using force sensor and the extra weight to be used in impedance control system and/or teleoperation system. 

Since there are high order nonholonomic constraints connecting the variables of the proposed non-redundant system, special treatment is needed to account for controlling the independent and dependent variables. 

The control objectives for the proposed robot can be divided into three main targets; robustness, optimal performance, and force estimation \& impedance control.

\subsubsection{Robustness}

Conventionally, robotic manipulators are controlled by using model based control methods such as feedback linearization, which is applied to the proposed system in \cite{new_quad_manp}. However, the conventional design methods are very sensitive to modeling errors which may lead to the degradation of system performance and stability. Model-free control methods have been proposed by using intelligent based control methods; however, they have a problem in real time implementation due to high computational cost. In \cite{khalifa2013adaptive}, Feedback Linearization, Direct Fuzzy Logic Control, and Fuzzy Model Reference Learning Control techniques have been applied to the proposed system. In the literature, several robust control methods have been proposed to improve the performance of robotic manipulators.
  
Disturbance Observer (DOb)-based controller is one of the most popular methods in the field of the robust motion control due to its simplicity  and computational efficiency. The motivation for using the DOb is to provide a robustness in front of a significant class of nonlinearities/uncertainties by estimating the nonlinear terms and external disturbances. Thus, one can solve the control problem relying on a set of linearized and decoupled Single Input Single Output (SISO) systems which are not affected by nonlinear/uncertain terms. As a result, a standard linear tracking controller can be used and the resulting control scheme is characterized by a low computational load with respect to the conventional nonlinear robust solutions.


The authors in \cite{kim2002performance, li2014disturbance} present the principles of DOb-based control system.  In the DOb  based  robust motion control systems, internal and external disturbances are observed by the DOb,  and  the  robustness is simply  achieved  by feeding-back the estimated disturbances in an inner-loop. Another  controller is designed in an outer loop so that the performance goals are achieved without considering  internal  and  external  disturbances. In \cite{Anal-servo-dis-obs}, the DOb-based controller is designed to realize a nominal system which can control acceleration in order to realize fast and precise servo system, even if servo system has parameter variation and suffers from disturbance. In \cite{choi2014simplified, hsia1988robust, murakami1993torque, wang2013trajectory, chen2014robust, eom2001disturbance, sariyildiz2015nonlinear}, DOb-based control technique has been applied to robotic systems and showed an efficient performance.


However, the previous work \cite{kim2002performance, li2014disturbance, sariyildiz2015nonlinear, eom2001disturbance, choi2014simplified, hsia1988robust, sariyildiz2015stability} in the DOb requires either the acceleration measurement or the velocity estimation. In fact, this is very difficult to be achieved and has limitations due to the available sensors for flying robots. In addition, it is feasible to measure the linear accelerations and angular velocities of the quadrotor via IMU while the angular velocities of the joints can be measured by encoders. Moreover, the estimation of the disturbances based on an estimated data (e.g., velocities), as in the case of the current developed DOb technique, will make the estimation error of these disturbances to be larger. In \cite{tomic2014unified}, the external wrench (i.e., external forces and moments) is estimated by using a model-based method for a simple UAV. In addition, the author utilizes the IMU data for the estimation. However, this method needs to know the dynamic model and it neglects some dynamics and nonlinearities. Also, it uses a nonlinear controller and estimates only the external disturbances without estimating the system dynamics. Thus, this technique is not a good choice for the considered aerial manipulator which is a high complex dynamic and kinematic robotic system. 


To cope up with these limitations, the conventional DOb is modified  to be compatible and feasible with the aerial manipulation system. The conventional DOb is redesigned and reformulated to use the linear acceleration and angular velocities data, which can be measured directly via the onboard IMU and encoders, to estimate the disturbances and nonlinearities.

\subsubsection{Optimal Performance}

MPC application to robotic systems in a true industrial environment, in which disturbances affect the robotic system and the model of the robot is inevitably inaccurate, is still limited. This is due to the high nonlinearities and uncertainties of dynamics in the robotics system. In \cite{hatanaka2009nonlinear, pin2009robust}, a nonlinear MPC is utilized to solve the problem of the control of highly nonlinear systems. In \cite{ferrara2013robust}, MPC control design with feedback linearization and sliding mode control are utilized to achieve robust trajectory tracking of robotic manipulator. In \cite{liu2011trajectory}, nonlinear MPC with nonlinear DOb is used to control a robotic system. However, the nonlinear control methods make the MPC to be more complex, has high computational cost, and is based on the knowledge of system model.

Based on the the linearization and robustness capabilities of the DOb, one can rely on the standard linear MPC methodology to design the controller of the outer loop of the DOb-based controller such that the system performance can be adjusted to achieve an objective tracking accuracy and speed. In addition, the actuators' constraints can be considered with optimal control effort and a low computational load.

\subsubsection{Sensorless Robust Force Estimation and Impedance Control}

Control of the interaction between a robot manipulator and the environment is crucial for successful execution of a number of practical tasks where the robot end-effector has to manipulate an object or perform some operation on a surface. Impedance control has the ability to impose, along each direction of the task space, a desired dynamic relation between the end-effector pose and the force of interaction with the environment (i.e., desired impedance). The inclusion of force information in the control of robots increases their adaptability to uncertain environments, such as those found in assembly tasks, and provides safety against breakage due to excessive contact forces \cite{seraji1997force, love1995environment, singh1995analysis}. Impedance control is still a rather far adopted solution in aerial robotics applications. In \cite{forte2012impedance, lippiello2012exploiting, lipiello2012cartesian, caccavale2008six}, an impedance control is designed for aerial manipulator without the need to measure/estimate the contact force. However, in such work, the authors neglect some dynamics as well as external disturbances. In addition, the proposed algorithm is model-based and it does not have a robustness capability. In \cite{hogan1987stable}, better results are obtained with feeding back the measured force when implementing impedance control. On the other hand, for the tele-manipulation, the use of force feedback is essential to assist the human operator in the remote handling of objects with a slave manipulator \cite{misra2006environment}. In addition, it is very critical to get the force feedback to achieve the cooperative grasping among aerial manipulation robots. If the load is heavier than the carrying capacity of a single UAV, multiple UAVs can distribute the load among them and move the object.

However, typically, forces are measured by a force sensor connected to the robot end-effector. This situation is infeasible in aerial robotics since force sensors have a lot of inherent limitations such as narrow bandwidth, sensing noise, and high cost. In addition, it needs complicated arrangements in the aerial manipulator that increase the weight which is a critical issue. Hence, to avoid a force sensor due to their limitations, the contact force has to be estimated. The estimated interaction force will be used in the impedance control algorithm and it can be utilized for tele-manipulation as well as for cooperative grasping for high payload transportation. 

Identification of the environment dynamics are more severe when the environment displays sudden changes in its dynamic parameters which cannot be tracked by the identification process. In \cite{hashtrudi1996adaptive}, it is found that in order to faithfully convey to the operator the sense of high frequency chattering of contact between the slave and hard objects, faster identification and structurally modified methods were required. Several techniques are proposed to estimate the contact force/environment dynamics. In \cite{sariyildiz2014guide}, the DOb and Recursive Least Squares (RLS) are used to estimate the environment dynamics. However, in this method, two DObs are used besides the RLS, and the estimation of contact force is activated only during the instance of contacting, thus there is a need to detect the instant at which the contact occurs. This  is not practical approach especially if one targets an autonomous system. In \cite{murakami1993force, eom1998disturbance, van2011estimating, phong2012external, colome2013external, alcocera2004force}, several techniques are proposed to achieve force control without measuring the force. However, these techniques are based on ignoring some dynamics and external disturbances, which will produce inaccurate force estimation. In \cite{ruggiero2014impedance}, a scheme is proposed which allows a quadrotor to perform tracking tasks without a precise knowledge of its dynamics and under the effect of external disturbances and unmodeled aerodynamics. In addition, this scheme can estimate the external generalized forces. However, as the authors claim, this estimator can work perfectly with constant external disturbances. Moreover, the estimated forces contain many different types such as wind, payload, environment impacts, and unmodeled dynamics. Thus, it cannot isolate the end-effector force alone from the others. The authors in \cite{tomic2014unified} present a model-based method to estimate the external wrench of a flying robot. However, this method assumes that there are no modeling errors and no external disturbance. Moreover, it estimates the external force as one unit and it can not distinguish between external disturbance and the end-effector force which is needed to calculate. In addition, it uses a model based control which needs a full knowledge of the model.     

  
Therefore, in this dissertation, another scheme is proposed to overcome these limitations of the currently developed techniques. Firstly, a DOb inner loop is used to estimate both the system nonlinearities and all external forces to compensate for them, as a result, the system acts like a linear decoupled SISO systems. Secondly, a fast tracking RLS algorithm is utilized with the linearization capabilities of DOb to estimate the contact force. Thirdly, a model-free robust impedance control of the quadrotor manipulation system is implemented. The DOb is designed in the quadrotor/joint space while the impedance control is designed in the task space such that the end-effector can track the desired task space trajectories besides applying a specified environment impedance. Thus, a Jacobian based algorithm is proposed to transform the control signal from the task space to the quadrotor/joint space coordinates.

\section{Objectives of Research}

Based on the reasoning in the previous section, this research proposes the control design and implementation of a new quadrotor manipulation system which will have great impacts in the human daily activities as well as other vital and critical applications.
  
The objectives of this research are clearly described as follows.

\subsection{Design and Modeling of the Quadrotor Manipulation System}

It is aimed to design a quadrotor with a 2-DOF manipulator that has a unique topology to enable the end-effector to track a desired 6-DOF trajectory. It has to provide solutions to limitations found on the currently developed aerial manipulation systems by having maximum mobility with minimum weight.

Kinematic and dynamic modeling of the system are aimed to facilitate designing and simulating the control of the system. 
 
\subsection{Experimental Setup and State Estimation}   

The whole system has to be built. An identification experiment is needed to find the actuators' coefficients. A measurement scheme is implemented to get the vehicle states (i.e., pose and velocity). Furthermore, this measurement scheme has to work in different places indoors and has potential to work outdoors as well.

Real time quadrotor/joint space control is designed, with a formulation that enables the system to work in either teleoperation or autonomous mode for pick and place operation.

An experimental test has to be carried out to demonstrate the feasibility and the effectiveness of the proposed approach with holding/releasing a payload.

\subsection{Inverse Kinematics} 

The proposed aerial manipulator has complexity in its inverse kinematics. In fact, inverse kinematics of the proposed system require a solution of complicated algebraic/differential equations to prove/achieve the end-effector ability to track arbitrary 6-DOF trajectories that lay within the capability of the used actuators. Therefore, in this work, a novel inverse kinematics algorithm is proposed, that solves the complex set of nonlinear differential algebraic equations approximately. This was not done before either for redundant or non-redundant aerial manipulator in the literature. After that, its accuracy has to be verified.

\subsection{Design of a Control Scheme} 

This robot has several issues in point of view of the control design, which have to be addressed and solved. In this research, a linear DOb-based control technique will be utilized as the base framework for the motion control. The DOb loop is used to enforce robust linear input/output behavior of the plant by canceling disturbances, measurement noise, and plant/model mismatch. The DOb loop has to use the measurements from the onboard sensors in order to reduce the disturbance estimation error.

To optimize the control signal, to save power consumption and thus increase mission time, and to consider the actuators' constraints, a MPC controller is designed in the external loop to achieve the required closed-loop performance.

Furthermore, the manipulation tasks require estimating (applying) a certain force at the end-effector as well as the accurate positioning of it. Thus, in this research, a robust force estimation and impedance control scheme is proposed. The robustness will be achieved based on the DOb technique. Then, a tracking linear impedance controller will be designed. Unlike the currently developed techniques for force estimation, a technique based on linearization capabilities of DOb and a Fast Tracking Recursive Least Squares (FTRLS) algorithm is proposed, which takes into consideration all the system dynamics with no need for the environment contact indication. 

\section{Thesis Contributions}
The added values of this thesis can be listed as following:

\begin{itemize}
	\item Developing a new non-redundant 6-DOF quadrotor-based aerial manipulation system that has superior features over the currently developed aerial manipulators.
	
	\item Experimental implementation of the proposed robot with the development of the measurement and estimation scheme to get the full state vector of the platform. This facilitates working within arbitrary places indoors as well as outdoors.
	 
    \item Proposing a novel inverse kinematics algorithm to prove the ability of the system to track arbitrary 6-DOF task space trajectories and facilitates designing the controller in the quadrotor/joint space. 
    
	\item Development of a control system for the proposed robot as follows:
	 
	\begin{itemize}
	\item Development of the Disturbance Observer technique to solve the robustness issue of this robot.
	
	\item Development of a robust optimal control based on the MPC and DOb approaches.
	
	\item Development of a robust sensorless force estimation and impedance control via the FTRLS and DOb techniques.
\end{itemize}
\end{itemize}

\section{Thesis Plan}

The Thesis is organized in 6 chapters as follows:

\textbf{Chapter 1} $\textendash$ Introduction. This chapter introduces the background and the objectives of the research. The outline of the thesis is also briefly described in this chapter.

\textbf{Chapter 2} $\textendash$ System Design and Modeling. This chapter initially describes the proposed flying robot. After that, the design of this system is presented. Then, the kinematic model is described. Finally, the system dynamics are reviewed.

\textbf{Chapter 3} $\textendash$ System Construction and Experiments. This chapter starts by describing the construction of the experimental system from point of view of both hardware and software. Then, it presents the identification experiment to get the rotors' aerodynamics parameters. After that, the 6-DOF system states measurements and estimation are presented. A PID controller with gravity compensation is designed and implemented in both simulation and experimental environments. The feasibility and effectiveness of the proposed system are verified by both simulation and experimental results.

\textbf{Chapter 4} $\textendash$ Inverse Kinematics Solution. This chapter presents a novel inverse kinematics analysis to get the reference quadrotor/joint space trajectories from desired 6-DOF task space trajectories. The accuracy of the proposed algorithm is enlightened via numerical results.

\textbf{Chapter 5} $\textendash$ Control System Development. This chapter describes the principles of the proposed DOb-based control system with a PD control in the outer loop. After that, the stability analysis of the closed-loop is presented. Then, it presents the application of an optimal robust control based on both DOb and MPC approaches. Moreover, presents the application of a robust sensorless force estimation and impedance control based on both DOb and FTRLS approaches. The effectiveness of the proposed methods are verified by simulation results.

\textbf{Chapter 6} $\textendash$ Conclusions. This chapter presents the overall conclusions of this
research work and describes the future developments of the research.


==> 5_motioncontrolscheme/motioncontrolscheme.tex <==
% this file is called up by thesis.tex
% content in this file will be fed into the main document

%: ----------------------- name of chapter  -------------------------
\chapter{\uppercase{Control System Development}} % top level followed by section, subsection
\label{ch:motioncontrolscheme}

%: ----------------------- paths to graphics ------------------------

% change according to folder and file names
\ifpdf
    \graphicspath{{5_motioncontrolscheme/figures/}}
\else
    \graphicspath{{5_motioncontrolscheme/figures/}}
\fi


%: ----------------------- contents from here ------------------------
This chapter proposes motion control systems to address and solve the control issues of the quadrotor manipulation system. These issues include; robust position control, robust optimal position control, and robust force estimation and impedance control.

The control of the quadrotor manipulation system is quite challenging because it is naturally unstable, and has strong nonlinearities. In addition, it is very susceptible to parameters variations due to adding/releasing the payload and the actuators' losses. Moreover, it is subjected to external disturbances like wind. Furthermore, its measurements are very noisy due to the thrusters that rotate at very high speed. Also, it has fast dynamics. Thus, there is a need to design and implement an efficient robust control technique to address these issues, which is presented in section \ref{se:pd_dob}. 

Furthermore, the actuators (thrusters and manipulator motors) have constraints, which may degrade the performance if it is not considered during controller design. Moreover, we have to apply an optimal control effort to reduce the required power of the thrusters such that we can save power and thus increase the mission time and/or increase the payload. Therefore, in section \ref{se:mpc_dob}, the Model Predictive Control (MPC) technique will be utilized based on the robust linearization capabilities of the DOb to address this issue.

Finally, in addition to the accurate positioning of the end-effector, the manipulation tasks require estimating (applying) certain force at the end-effector as well.. Thus, in section \ref{se:ftrls_dob}, a robust force estimation and impedance control scheme is proposed. The robustness will be achieved based on the DOb technique. Then, a linear impedance controller will be designed in the joint space. The contact force is be identified based on robust linearization capabilities of DOb and a Fast Tracking Recursive Least Squares (FTRLS) algorithm, which takes into consideration all the system dynamics with no need for the environment contact indication. 
%----------
%: -------- end of thesis sub-document -----------
\section{Control Objectives} \label{sse:cntrl_obj}

We target the design of the control system in order to satisfy the following objectives:

\begin{objective} \label{obj:stab} 
	(Robust Stability) The considered robotic system is stable and robust in the presence of the external disturbances, uncertainties, and noises.
\end{objective}

\begin{objective} \label{obj:track} (Trajectory Tracking)
	$6$-DOF task space trajectory tracking is achieved.
\end{objective}

\begin{objective} \label{obj:optimal} (Optimal Performance)
	Minimization of the controller efforts, and constraints them to be within the allowable limits of the system actuators (i.e., thrust forces and motor's torques).
\end{objective}

\begin{objective} \label{obj:force} (Force Estimation) The end-effector contact force has to be estimated fast.
\end{objective}

\begin{objective} \label{obj:impd}($6$-DOF Impedance Control) In the presence of the contact force, desired impedance at the end-effector is achieved.
\end{objective}

\section{Robust Position Control} \label{se:pd_dob}

In this section, a modified version of the well-known Disturbance Observer-based robust control is proposed  in order to achieve the robust 6-DOF task space trajectory tracking against the system nonlinearities, couplings, uncertainties,  disturbances, and measurement noise.

To achieve control objectives \ref{obj:stab} and \ref{obj:track}, a control technique as shown in Fig. \ref{fig:pd_dob_fncblg} is proposed. In this strategy, the system nonlinearities, uncertainties, external disturbances, $\tau^{dis}$, are treated as extended disturbances which will be estimated, $\hat{\tau}^{dis}$, and canceled by the DOb in the inner loop. The system can be now considered as linear SISO plants, and thus,  simple PD controller is used in the external loop to achieved the target performance for the system by producing $\tau^{des}$. Another loop is presented to find the desired quadrotor/joint space trajectories from the target $6$-DOF task space based on the inverse kinematic analysis that is presented in chapter \ref{ch:InverseKinematics}. Hence, the controller can be designed in the quadrotor/joint space. 
%===================================================
\begin{figure}[h]
	\centering
	\includegraphics[width=1\textwidth]{pd_dob_fncblg}
	\caption{Functional block diagram of the proposed PD-DOb control system}
	\label{fig:pd_dob_fncblg}
\end{figure}
%===================================================
\subsection{DOb-based Controller}

Disturbance Observer (DOb)-based controller is one of the most popular methods in the field of robust motion control due to its simplicity  and computational efficiency.  In  DOb-based  robust motion control systems, internal and external disturbances are observed by the DOb,  and the  robustness is simply  achieved  by feeding-back the estimated disturbances in an inner-loop. Another  controller is designed in an outer loop so that the performance goals are achieved without considering  internal  and  external  disturbances. 


A block diagram of the conventional DOb inner loop is shown in Fig. \ref{fig:interlp_DOb_vel}. In this figure, $M_n$ $\in \mathbb{R}^{8 \times 8}$ is the system nominal inertia matrix, $\tau^{des}$ is the desired input vector, $P=diag([g_1,...,g_i,...,g_8])$ with $g_i$ is the bandwidth of the low pass filter of the $i^{th}$ variable of $q$, $Q(s)=diag([\frac{g_1}{s+g_1} ,...,\frac{g_i}{s+g_i},...,\frac{g_8}{s+g_8}])$ $\in \mathbb{R}^{8 \times 8}$ is the matrix of the low pass filter of DOb. The DOb requires velocity measurements. 
%Practically, the velocity have to be fed through a low pass filter, $Q_v(s)=diag([\frac{g_{v_1}}{s+g_{v_1}},...,\frac{g_{v_i}}{s+g_{v_i}},...,\frac{g_{v_8}}{s+g_{v_8}}])$ $\in \mathbb{R}^{8 \times 8}$, and with cut-off frequency of $P_v=diag([g_{v_1},...,g_{v_i},...,g_{v_8}])$ (i.e. velocity measurement is achieved in a predetermined bandwidth). 
$\tau^{dis}$ represents the system extended disturbances including the Coriolis, centrifugal and gravitational terms, and external disturbances, and $\hat{\tau}^{dis}$ represents the system estimated disturbances. $K$ is the external controller that is used to achieve the required control performance.

If  one can  apply  the  concept  of  disturbance  observer to the proposed system, then the independent coordinate  control is possible  without  considering the coupling effect of the other coordinates. The  coupling  terms  such  as centripetal  and  Coriolis and gravity terms are considered as disturbance and compensated by feeding back the estimated disturbance torque. 

%=========================
\begin{figure}[h]
	\centering
	\includegraphics[width=1\columnwidth]{interlp_DOb}
	\caption{Block diagram of the conventional DOb internal loop}
	\label{fig:interlp_DOb_vel}
\end{figure}
% ===========================================
As we noted in this structure, the DOb utilizes the estimated velocity measurement to estimate the system disturbances.

However, it is well known that the linear accelerations and angular rates of the quadrotor can be measured directly from the IMU. In addition, the angular velocities of the joints can be measured via an encoder. Therefore, a block diagram of the modified DOb-based controller is proposed as in Fig. \ref{fig:DOb-str} for our robotic system. In this modified DOb-based control, two different DOb loops are used. One is based on the measured  accelerations, while the other is based on the measured velocities.

%=========================
\begin{figure}
	\centering
	\includegraphics[width=1\textwidth]{DOb-str_new}
	\caption{Block diagram of the modified DOb-based controller}
	\label{fig:DOb-str}
\end{figure}
% ===========================================

In this figure, $M_n = \begin{bmatrix} M_{n_a} & O_{3 \times 5} \\ O_{5 \times 3} & \ M_{n_v}\end{bmatrix}$ $\in \mathbb{R}^{8 \times 8}$ is the system nominal inertia matrix with $M_{n_a}$ $\in \mathbb{R}^{3 \times 3}$ represents the nominal inertia for the translational coordinates, ${p}_b$, while $M_{n_v}$ $\in \mathbb{R}^{5 \times 5}$ represents the nominal inertia for the rotational coordinates, ${\Phi}_b$ and ${\Theta}$. $Q_a(s)=diag([\frac{g_1}{s+g_1} \ ... \ \frac{g_3}{s+g_3}])$, and $Q_v(s)=diag([\frac{g_4}{s+g_4} \ ... \ \frac{g_8}{s+g_8}])$ are the matrices of the low pass filter of DOb for the translational and rotational coordinates, respectively. $P_a=diag([g_1 \ g_2 \ g_3])$ and $P_v=diag([g_4 \ ... \ g_i \ ... \ g_8])$ vectors of bandwidths of the DOb filter  for translational and rotational coordinate, respectively. $\tau= [\tau_a^T \ \tau_v^T]^T$ represents the robot's generalized forces for the translational and rotational coordinates. $\hat{\tau}^{dis} = [\hat{\tau}_a^{{dis}^T} \ \hat{\tau}_v^{{dis}^T}]^T$ represents the system estimated disturbances. 

The system disturbance, $\tau^{dis}$, can be calculated as
\begin{equation}
\begin{split}
\tau^{dis} = (M(q) - M_n) \ddot{q} + \tau^d,\\ 
\tau^d=C(q,\dot{q}) \dot{q} + G(q) + d_{ex}.
\label{eq:sys_dis}
\end{split}
\end{equation}  
The control input, $\tau$, in Fig. \ref{fig:DOb-str} can be calculated as
\begin{equation}
\tau = M_n \ddot{q}^{des} + \hat{\tau}^{dis},
\label{eq:tau1}
\end{equation}  
where
\begin{equation}
\hat{\tau}^{dis} = Q (\tau - M_n \ddot{q}).
\label{eq:tau_dis_est}
\end{equation}
 
Thus, the control input, $\tau$, can be calculated as
\begin{equation}
\begin{split}
\tau =  M_n \ddot{q}^{des} + M_n P e_v,
\label{eq:tau}
\end{split}
\end{equation}  

where $e_v = \dot{q}^{des} - \dot{q}$, and $\ddot{q}^{des}$ that is the output from the outer loop controller which will be designed later.

By the virtue that the DOb works ideal, then
\begin{equation}
\hat{\tau}^{dis} = \tau^{dis}. 
\label{eq:tau_hat}
\end{equation}

Thus, the dynamics from the DOb loop input $\tau^{des}$ to the output of the robot manipulator are given by
\begin{equation}
M_n \ddot{q}^{des}=\tau^{des}.
\label{eq:sys_eq_reduced}
\end{equation}
Since $M_n$ is chosen to be a diagonal matrix, the system can be treated as multi-decoupled linear SISO systems as
\begin{equation}
M_{n_{ii}} \ddot{q}_i^{des}=\tau_i^{des},
\label{eq:sys_eq_decoupled}
\end{equation}
or simply in the acceleration space as
\begin{equation}
\ddot{q}_i=\ddot{q}_i^{des}.
\label{eq:sys_eq_decoupled_acc}
\end{equation}
All that remains in the design of the DOb based controller is the design of the tracking controller, $K(s)$, in the DOb outer loop. A PD-based tracking controller for the system of (\ref{eq:sys_eq_decoupled_acc}) is chosen as
\begin{equation}
\ddot{q}^{des} = \ddot{q}_{r} + K_P (q_r - q) + K_D (\dot{q}_r - \dot{q}),
\label{eq:ext_ctrl}
\end{equation}

where $K_P$ and $K_D$ $\in R^{8 \times 8}$ are the proportional and derivative
gains of the PD controllers, receptively. $q_r$, $\dot{q}_{r}$, and $\ddot{q}_{r}$ are the references for linear/angular positions, velocities, and accelerations, respectively. By proper selection of $K_P$ and $K_D$, one can tune the response of the  the error dynamics as necessary.

To ensure that the system stability under this control can be guaranteed, we do the following analysis.
	
The control law in (\ref{eq:tau}) leads to the following error dynamics
	\begin{equation}
	\begin{split}
	M(q) \dot{e}_v + C(q,\dot{q}) e_v +  K_v e_v = \delta, 
	\\ K_v = P M_n,
	\label{eq:dyn_gen_dobeD}
	\end{split} 
	\end{equation} 
	and
	\begin{equation}
	\dot{e} + K_D e  + K_P \int e \ dt = e_v,  
	\label{eq:ext_ctrl_err}
	\end{equation}
	where
	\begin{equation}
	\delta = \Delta M(q) \ddot{q}^{des} + C(q,\dot{q}) \dot{q}^{des} + G(q) + d_{ex}, 
	\label{eq:delta}
	\end{equation} 
	and $\Delta M(q) = M(q) - M_n$.
	
	Equation (\ref{eq:dyn_gen_dobeD}) represents the error dynamics of the DOb loop.
	
Let us assume the following Lyapunov function
	\begin{equation}
	V=\frac{1}{2} e_v^T M(q) e_v.
	\label{eq:lyp_fun}
	\end{equation} 
	The time derivative of this function is
	\begin{equation}
	\dot{V}= e_v^T M(q) \dot{e}_v + \frac{1}{2} e_v^T \dot{M}(q) e_v.
	\label{eq:lyp_der1}
	\end{equation} 
	Substituting from (\ref{eq:dyn_gen_dobeD}), then (\ref{eq:lyp_der1}) becomes
	\begin{equation}
	\dot{V}= e_v^T \delta - e_v^T K_v e_v + \frac{1}{2} e_v^T (\dot{M}(q) - 2 C(q,\dot{q}))e_v.
	\label{eq:lyp_der2}
	\end{equation} 
	The dynamic equation of motion (\ref{eq:dyn_gen}) posses several well known properties \cite{from2014vehicle, spong2006robot}.
	
	\begin{property}
		\begin{equation}
		\lambda_{min} \norm{\nu}^2  \leq  \nu^T M(q) \nu \leq \lambda_{max} \norm{\nu}^2 
		\label{eq:M_pro}
		\end{equation}
	\end{property}
	
	\begin{property}
		\begin{equation}
		\nu^T(\dot{M}(q) - 2 C(q,\dot{q}))\nu=0
		\label{eq:d/dt_pro}
		\end{equation} 
	\end{property}
	where $\dot{M}(q) - 2 C(q,\dot{q})$ is a skew-symmetric matrix, $\nu \in \mathbb{R}^8$ represents a $8$-dimensional vector, and $\lambda_{min}$ and $\lambda_{max}$ are positive real constants that are the minimum and maximum eigen values of the matrix $M(q)$, respectively. 
	
	Substituting from (\ref{eq:d/dt_pro}) into (\ref{eq:lyp_der2}), then (\ref{eq:lyp_der2}) will be
	\begin{equation}
	\dot{V}= e_v^T \delta - e_v^T K_v e_v. 
	\label{eq:lyp_der3}
	\end{equation}
	
	From the robot dynamic property (\ref{eq:M_pro}), one can find:
	\begin{equation}
	\dot{V} \leq -\gamma V + \sqrt{\frac{2 V}{\lambda_{min}}} |\delta|,
	\label{eq:lyp_der4}
	\end{equation}
	where $\gamma = \frac{2K_v}{\lambda_{max}}$.
	
From the analysis presented in \cite{sadegh1990stability, bickel1999passivity}, we complete the analysis as following.

Dividing (\ref{eq:lyp_der4}) by $V^{0.5} \neq 0$ will give

	\begin{equation}
	\frac{d}{dt}(V^{0.5}) + 0.5 \gamma V^{0.5}  \leq \sqrt{\frac{2}{\lambda_{min}}} |\delta|,
	\label{eq:lyp_der5}
	\end{equation}

By multiplying (\ref{eq:lyp_der5}) by $e^{-0.5 \gamma}$ and integrating, then we get
	\begin{equation}
	V^{0.5} \leq e^{-0.5 \gamma t} V^{0.5}(0,e_v(0)) + V_c,
	\label{eq:lyp_der6},
	\end{equation}
with 
	\begin{equation}
	V_c = \frac{1}{\sqrt{2 \lambda_{min}}} \int_{0}^{t} e^{-0.5 \gamma (t-\iota)} |\delta(\iota)| d \iota. 
	\label{eq:lyp_der7}
	\end{equation}
One can rewrite $V_c$ as
	\begin{equation}
	V_c =  \frac{1}{\sqrt{2 \lambda_{min}}} (e^{-0.5 \gamma t} * |\delta(t)|).
	\label{eq:lyp_der8}
	\end{equation}
Taking the $\norm{.}_p$, gives
	\begin{equation}
	\norm{V_c}_p = \frac{1}{\sqrt{2 \lambda_{min}}} \norm{e^{-0.5 \gamma t} * \delta(t)}_p.
	\label{eq:lyp_der9}
	\end{equation}  
\begin{lemma}(\cite{desoer2009feedback}) \label{lm:1}
Consider $\varUpsilon_1 \in L_1$, $\varUpsilon_2 \in L_p$, then
\begin{equation}
\norm{\varUpsilon_1 * \varUpsilon_2}_p \leq \norm{\varUpsilon_1}_1 \norm{\varUpsilon_2}_p.
\end{equation} 
\end{lemma}	
	
From $Lemma$ \ref{lm:1}, then (\ref{eq:lyp_der9}) is

	\begin{equation}
	\norm{V_c}_p = \frac{1}{\sqrt{2 \lambda_{min}}} \norm{e^{-0.5 \gamma t}}_1 \norm{\delta(t)}_p,
	\label{eq:lyp_der10}
	\end{equation}
but $\norm{e^{-0.5 \gamma t}}_1$ = $0.5 \gamma$, so 
	\begin{equation}
	\norm{V_c}_p = 0.5 \gamma \frac{1}{\sqrt{2 \lambda_{min}}}  \norm{\delta(t)}_p.
	\label{eq:lyp_der11}
	\end{equation}
Thus, (\ref{eq:lyp_der6}) is
	\begin{equation}
	\norm{V^{0.5}}_p \leq \norm{e^{-0.5 \gamma t} V^{0.5}(0,e_v(0))}_p + 0.5 \gamma \frac{1}{\sqrt{2 \lambda_{min}}}  \norm{\delta(t)}_p.
	\label{eq:lyp_der12}
	\end{equation}
This expression (\ref{eq:lyp_der12}) can be simplified to be

\begin{equation}
\norm{e_v}_p \leq \frac{1}{\gamma} + \sqrt{\frac{2}{\lambda_{min}}} (\frac{2}{p\gamma})^{\frac{1}{p}} \sqrt{V(0,e_v(0))} \norm{\delta}_p.
\label{eq:ev_final}
\end{equation}

Thus, the error dynamics is $L_p$ input/output stable with respect to the pair ($\delta$, $e_v$) for all $p \in [1,\infty)$. 
\begin{lemma}(\cite{ioannou2012robust}) \label{lm:2}
	Let
	\begin{equation}
	e = H_{PD}(s) e_v,
	\label{eq:lemma_1}
	\end{equation}
	where $H_{PD}(s)$ is an strictly proper and exponentially stable transfer function. Then $e_v \in L_p$ implies that $e \in L_p$ and $\dot{e} \in L_p$. 
\end{lemma}
Form (\ref{eq:ext_ctrl_err}), the transfer function between $e$ and $e_v$ is proper exponentially stable as long as the parameters $K_P$ and $K_D$ are positive definite matrices. Therefore, Lemma \ref{lm:2} implies that both $e$ and $\dot{e}$ $\in L_p$.	
\begin{remark}
	Equation (\ref{eq:lyp_der4}) indicates that the convergence rate increases proportionally with $K_v$. However, we have to take into considerations the constraints on $g_i$ due to the sampling time.
\end{remark}

Fig. \ref{fig:kin_cform_block} presents the detailed block diagram of the proposed motion control system based on the inverse kinematic analysis and on the DOb quadrotor/joint space-based control. The desired trajectories for the end-effector's position and orientation $\chi_{e,r} (t)$, $p_{e,r}(t)$ and $\Phi_{e,r}(t)$, are fed to the inverse kinematic algorithm together with $\sigma_{b,r}(t)$ generated from the nonholonomic constraints such that the desired trajectories in vehicle/joint space, $\zeta_r(t)$, are obtained. After that, the controller block receives the desired trajectories and the feedback signals from the system and provides the control signal, $\tau$ $=$ $B u$.
%=================================
\begin{figure}
	\centering
	\includegraphics[width=1\textwidth]{kin_cform_block}
	\caption{Detailed block diagram of the PD-DOb control system}
	\label{fig:kin_cform_block}
\end{figure}
%=================================

Since the linear position, joints angles, and the yaw angle are usually the controlled variables while pitch and roll angles are used as intermediate control inputs for horizontal position control, the proposed control system consists from two DOb-based controllers; one for $\zeta$ (with $K_{\zeta}(s)$, $M_{n_a}$, $M_{nv_1}$ ,$P_{v_1}$, $Q_{v_1}$, and $Q_{a}$) and the other for $\sigma_b$ (with $K_{\sigma}(s)$, $M_{nv_2}$, $P_{v_2}$, $Q_{v_2}$). 

The desired values $\sigma_{b,r}$ for the intermediate controller are obtained from the output of position controller, $\tau_{\zeta}$, through the relation
\begin{equation}
\sigma_{b,r} = \frac{1}{\tau_{\zeta}(3)}
\begin{bmatrix}
C_{\psi} & S_{\psi} \\
S_{\psi} & -C_{\psi} 
\end{bmatrix}
\begin{bmatrix}
\tau_{\zeta}(1) \\
\tau_{\zeta}(2) 
\end{bmatrix} 
\label{eq:sigmad},
\end{equation} 
which can be derived from (\ref{eq:Rb}) based on small angle approximation.

The desired value of the pitching and rolling, $\sigma_{b,r}$, is then fed back to the inverse kinematics algorithm.

The output of the two controllers, $\tau_{\zeta}$ and $\tau_{\sigma}$, are mixed to generate the final control vector $\tau$ which is converted to the forces/torques applied to quadrotor/manipulator by
\begin{equation}
u= B_6^{-1} \begin{bmatrix}
\tau_{\zeta}(3,4)\\
\tau_{\sigma}\\
\tau_{\zeta}(5,6) 
\end{bmatrix},  
\label{eq:ufinal}
\end{equation}
where $B_6$ $\in \mathbb{R}^{6 \times 6}$ is part of $B$ matrix and it is given by $B_6 = B(3:8,1:6)$.

\begin{remark}
	It is noted from the quadrotor dynamics \cite{hua2013introduction, isidori2012robust, choi2015nonlinear} that the response of the intermediate, $\sigma$, controller must be faster than that of the position control loop. However, as stated in the above analysis, the convergence rate of errors dynamics ($e_v$ and $e$) is directly proportional to the $K_v$, $K_P$, $K_D$. Therefore, we have to tune $K_v$, $K_P$, and $K_D$, such that the response speed of $\sigma_b$ is much faster than that of $\zeta$. 
\end{remark}

\subsection{Simulation Study} \label{se:sim_dob}

In this section, the previously proposed control strategy is simulated in MATLAB/SIMULINK program for the considered aerial manipulation system.

\subsubsection{Simulation Environment} \label{se:sim_dob_envirnemnt}
In order to make the simulation quite realistic, the
following setup and assumptions have been made:
\begin{itemize}
	\item The model has been identified on the basis of real data through experimental tests. The identified parameters are given in Table \ref{tab:sys_par}.
	\item Linear and angular position and velocity of the quadrotor are available at rate of $1$ kHz.
	\item The position and velocity of the manipulator joints are available at rate of $1$ kHz.
	\item A normally distributed measurement noise, with mean of $10^{-3}$ and standard deviation of $5 \times 10^{-3}$, has been added to the measured signals.
	\item The controller outputs are computed at a rate of $1$ kHz.
	\item  In order to test the robustness to the model
	uncertainties, a step change is introduced, at instant $15$ s, in the control matrix, $N$, which can simulate sudden actuators' losses, whose elements are assumed to be equal to 0.9 times their true values (i.e., $10 \% $ error).
	\item The end-effector has to pick a payload of value $200$ g at instant $20$ s and release it at $40$ s.
\end{itemize}

\subsubsection{Results and Discussion}

Tables \ref{tab:DOb_par_jonit} presents the controller parameter for the proposed control technique. The reference trajectories for the end-effector are chosen such that the end-effector moves on a circular helix, while its orientation follows quintic polynomial trajectories.

The simulation results are presented in Figs. \ref{fig:kin_ee_cform_results}, \ref{fig:kin_joint_cform_results} and \ref{fig:kin_cform_results_3D}. From these figures, it is possible to recognize that there are small oscillations after starting the system operation due to the time needed to estimate the nonlinearities and disturbances. This time is about $4$ s. After this period, the controller can quickly recover this error and provides good tracking of the desired trajectories. Moreover, it is clear that the capability of the controller to recover, with fast response (about $0.05$ s), the tracking error due to the presence of the payload and the uncertainty in system parameters. Moreover, Fig. \ref{fig:kin_joint_cform_results} indicates that the quadrotor/joint space trajectories are within the allowable limits of the joints (270$^{\circ}$). Furthermore, Fig. \ref{fig:kin_cform_results_omega} indicates that the required actuators efforts, which are the required thrust force from each rotor and the torque from each manipulator's motor, $u$, are in the allowable limit. The maximum thrust force for each rotor is $8$ N as obtained from the identification process, while the allowable input torque for the motor of joint $1$ is $0.7$  N.m and $0.4$  N.m for that of joint $2$ as stated in the motors' data sheet. Therefore, one can contend that the control objectives \ref{obj:stab} and \ref{obj:track} are achieved by using this motion control scheme.
%============================================
\begin{table}[!h]
	\caption{PD-DOb parameters}
	\label{tab:DOb_par_jonit}
	\begin{center}
		\setlength{\tabcolsep}{1pt}
		\begin{tabular}{|c|c|c|c|c|c|}
			\hline
			Par. & Value & Par. & Value \\
			\hline
			$M_{n_\zeta}$	& $diag\{1.2, 1.2, 1.2, 0.02, 0.004, 0.0009\}$ & $M_{n_\sigma}$ & $diag\{0.02, 0.02\}$ \\
			\hline
			$K_{P_\zeta}$	& $diag\{3,3,10,3,3,3\}$& $K_{P_\sigma}$ & $diag\{10, 10\}$\\
			\hline
			$K_{D_\zeta}$	& $diag\{1.5,1.5,5,3,3,3\}$& $K_{D_\sigma}$ & $diag\{7, 7\}$\\
			\hline
			$P$ &  \multicolumn{2}{c}{$[10 \ 10 \ 10 \ 100 \ 100 \ 100 \ 100 \ 100]^T$}&\\
			\hline
		\end{tabular}
	\end{center}
\end{table}
%============================================
\begin{figure}[!h]
	\centering
	\begin{tabular}{cc}
		\subfloat[$x$]{\includegraphics[width=0.4\columnwidth]{x_traj_IK_dob}}&
		\subfloat[$y$]{\includegraphics [width=0.4\columnwidth]{y_traj_IK_dob}}\\
		\subfloat[$z$]{\includegraphics [width=0.4\columnwidth]{z_traj_IK_dob}}&
		\subfloat[$\psi$]{\includegraphics [width=0.4\columnwidth]{ep_traj_IK_dob}}\\
		\subfloat[$\theta_{1}$]{\includegraphics [width=0.4\columnwidth]{th1_traj_IK_dob}}&
		\subfloat[$\theta_{2}$]{\includegraphics [width=0.4\columnwidth]{th2_traj_IK_dob}}
	\end{tabular}
	\caption{PD-DOb results: The actual response in the quadrotor/joint space; a) $x$, b) $y$, c) $z$, d) $\psi$, e) $\theta_{1}$, and f)  $\theta_{2}$}
	\label{fig:kin_joint_cform_results}
\end{figure}
%============================================
\begin{figure}[!h]
	\centering
	\begin{tabular}{cc}
		\subfloat[$x_{e}$]{\includegraphics[width=0.4\columnwidth]{xe_traj_IK_dob}}&
		\subfloat[$y_{e}$]{\includegraphics [width=0.4\columnwidth]{ye_traj_IK_dob}}\\
		\subfloat[$z_{e}$]{\includegraphics [width=0.4\columnwidth]{ze_traj_IK_dob}}&
		\subfloat[$\phi_{e}$]{\includegraphics [width=0.4\columnwidth]{phe_traj_IK_dob}}\\
		\subfloat[$\theta_{e}$]{\includegraphics [width=0.4\columnwidth]{the_traj_IK_dob}}&
		\subfloat[$\psi_{e}$]{\includegraphics [width=0.4\columnwidth]{epe_traj_IK_dob}}
	\end{tabular}
	\caption{PD-DOb results: The actual response of the end-effector pose; a) $x_{e}$, b) $y_{e}$, c) $z_{e}$, d) $\phi_{e}$, e) $\theta_{e}$, and f) $\psi_{e}$. The inner box of each figure represents zooming on that figure from instant 0 s to instant 5 s.}
	\label{fig:kin_ee_cform_results}
\end{figure}
%==============================================
\begin{figure}[!h]
	\centering
	\includegraphics[width=0.5\columnwidth]{3D_traj_IK_dob}
	\caption{PD-DOb results: 3D trajectory of end-effector with fixed orientation (The marker represents the end-effector orientation; Green, Blue, and Red for x-,y, and z-axis)}
	\label{fig:kin_cform_results_3D}
\end{figure}
%=================================
\begin{figure}[!h]
	\centering
	\includegraphics[width=0.9\columnwidth]{OM_traj_IK_dob}
	\caption{PD-DOb results: The required control efforts}
	\label{fig:kin_cform_results_omega}
\end{figure}
%=====================================
\clearpage
\section{Robust Optimal Position Control} \label{se:mpc_dob}
In this section, based on the robust linearization capabilities of the DOb that presented in the previous section, the continuous MPC \cite{wang2009model} technique will be used to achieve an optimal performance for the aerial manipulator, in addition to keep the actuators's inputs within their limits.

To achieve the control objectives \ref{obj:stab} - \ref{obj:optimal}, a control technique as shown in Fig. \ref{fig:mpc_dob_fncblg} is proposed. In this strategy, the system nonlinearities, uncertainties, external disturbances, $\tau^{dis}$, are treated as extended disturbances which will be estimated, as $\hat{\tau}^{dis}$, and canceled by the DOb in the inner loop. The system can be now considered as linear SISO subsystems, and thus, the MPC is used in the external loop to achieve the target performance for the system by producing $\tau^{des}$. Another loop, inverse kinematics, is presented to find the desired quadrotor/joint space trajectories from the target $6$-DOF task space trajectory. 
%===================================================
\begin{figure}
	\centering
    \includegraphics[width=0.7\textwidth]{mpc_dob_fncblg}
	\caption{Functional block diagram of the proposed MPC-DOb control system}
			\label{fig:mpc_dob_fncblg}
\end{figure}
%===================================================

\subsection{Linearized Model}
 
By virtue of the rejection of the nonlinearities, disturbances, uncertainties, and noise by the usage of DOb internal loop as presented in section \ref{se:pd_dob}, the MPC controller has not to consider uncertainties and can be designed based on the nominal $8$ SISO decoupled  models of the system with satisfying the actuators' constraints, $u^{min}$ $\leq$ $u$ $\leq$ $u^{max}$. However, in determining $u^{max}$ and $u^{min}$, the contribution of $\hat{\tau}^{dis}$ should be considered.  

The state space SISO model of the system of (\ref{eq:sys_eq_decoupled_acc}) is
\begin{align}
	\dot{x}_p(t) = A_p x_p(t) + B_p u_{mpc}(t), \nonumber \\
	q_i(t) = C_p x_p(t), 
	\label{eq:siso}
\end{align}
where
$x_p= \begin{bmatrix}
x_1  \\
x_2  \\
\end{bmatrix} = 
\begin{bmatrix}
q_i  \\
\dot{q}_i\\
\end{bmatrix}$,
$A_p= \begin{bmatrix}
0 & 1 \\
0 & 0 \\
\end{bmatrix}$, 
$B_p= \begin{bmatrix}
0  \\
1  \\
\end{bmatrix}$,
$C_p= \begin{bmatrix}
1 & 0 \\ 
\end{bmatrix}$, 
and $u_{mpc}(t)$ is the output of the external controller, MPC, which will be $\ddot{q}^{des}_i$.

\subsection{Continuous time MPC}

The MPC can be designed in continuous time or discrete time models. One of the key advantages in using continuous time predictive control instead of discrete-time predictive control is that the design model and the algorithm are robust in a fast sampling environment. The discrete-time models and predictive control algorithms could encounter problems when the system is under fast sampling condition. Another advantage is that because the design is performed in the continuous-time domain, the discretization is carried out in the implementation stage and the framework permits the control of an irregular sampled-data system. Thus, the continuous time MPC will be used in this research. 

The general design philosophy of model predictive control is to compute a trajectory of a future manipulated variable, $u_{mpc}(t)$, to optimize the future behavior of the plant output $q_i(t)$. In other words, the MPC uses a dynamical model of the process to predict its future evolution and optimize the control signal. The optimization is performed within a limited time window starts by $t_i$ with length $T_p$. With a given initial time $t_i$, the window is taken from $t_i$ to $t_i$ + $T_p$. The length of the window $T_p$ remains constant. The prediction horizon equals
the length of the moving horizon window $T_p$ and indicates how far the future will be predicted. Thus, it provides the advantage of repeated online optimization. Based on the receding horizon control principle, although the optimal
trajectory of the future control signal is completely captured within the moving horizon window, the actual control input to the plant only takes the first
instant of the control signal, while neglecting the rest of the trajectory. At a given time, the first value of this optimal sequence is applied to the process. When a new set of measurements is available to the controller, a re-optimization is performed, and the first value of this new optimal sequence of manipulated variables is implemented. 

%However, the control trajectory is required to satisfy the property that its integral squared value is bounded as
%\begin{equation}
%\int_{0}^{\infty} u_{mpc}(t)^2 \ dt < \infty
%\label{eq:u_bound}
%\end{equation}
%
%It is a fact that if there is an external constant input signal to the control system, such as a set-point signal or a constant disturbance signal, the control signal itself does not satisfy (\ref{eq:u_bound}). This is because in order to follow the set-point signal, the control signal needs to converge to a non-zero constant that is related to the steady-state gain of the plant and the magnitude of the set-point
%change. Therefore, instead of modeling the control signal, 

The continuous-time MPC design \cite{wang2009model} uses the derivative of the control signal, $\dot{u}_{mpc}(t)$, and thus it is always designed based on an augmented model of the plant which is given by
%which will satisfy the property,
%\begin{equation}
%\int_{0}^{\infty} \dot{u}_{mpc}(t)^2 \ dt < \infty.
%\label{eq:ud_bound}
%\end{equation}
%This implies that the he signal $\dot{u}_{mpc}(t)$ is an exponentially decay function that goes to $\infty$ (i.e., $\int_{0}^{\infty} \dot{u}_{mpc}(t)^2 \ dt < \infty$). 

%Therefore, the MPC will be designed based on an augmented model of the plant which is given by
\begin{equation}
	\begin{split}
		\dot{x}_a(t) = A_a x_a(t) + B_a \dot{u}_{mpc}(t), \\
		q_i(t) = C_a x_a(t), 
		\label{eq:aug_siso}
	\end{split}
\end{equation}
where
$
x_a(t)= \begin{bmatrix}
\dot{x}_p(t) \\
q_i(t)  
\end{bmatrix}
$,
$
A_a= \begin{bmatrix}
A_p & O_{2\times1} \\
C_p & 1 
\end{bmatrix}
$, 
$
B_a= \begin{bmatrix}
B_p  \\
0  
\end{bmatrix} 
$,
$
C_a= \begin{bmatrix}
O_{1\times2} & 1  
\end{bmatrix}. 
$
This implies that the signal $\dot{u}_{mpc}(t)$ is an exponentially decay function that goes to 0. 
%When designing a continuous-time model predictive control system, the trajectories of the future control
%signals need to be described using orthonormal basis functions so that the optimization problem is converted to finding a set of coefficients that will minimize an objective function subject to constraints
%(see Wang (2009)).

%Because of the orthonormal properties and completeness of the Laguerre functions, their applications in
%continuous-time model predictive control will ensure that the predictive control trajectories will converge
%to the underlying optimal control trajectories as the numbers (N1, N2) of Laguerre functions increase.

%This augmented model adds an integrator to the MPC design. The integral action removes both the small linearization error (i.e., DOb estimation error) and measurement noises. 

%In addition, it enables the model to use the derivative of the control as its input signal, while maintaining the same output.
 
Therefore, the control trajectory, $\dot{u}_{mpc}(t)$, can be modeled by a set of exponentially decaying functions within the interval
$0 \leq \iota \leq T_p$.

% which satisfies
%\begin{equation}
%\lim\limits_{T_p \longrightarrow \infty}  \int_{0}^{T_p} \dot{u}_{mpc}(\iota)^2 \ d \iota < \infty.
%\label{eq:fnc_bound}
%\end{equation}
One candidate function, to describe the derivative of the control signal, is the set of Laguerre polynomials \cite{wang2001continuous, barry2004model}, which is a set of orthonormal functions. 
 
The following set of Laguerre functions is used
 \begin{align}
 X(t) = X(0) e^{A_u t}, 
 \label{eq:l_fnc}
 \end{align}
 where  
 $
 A_u= \begin{bmatrix}
 -s_u & 0 & ... & 0\\
 -2s_u & -s_u & ... & 0\\
 ... & ... & ... & ...\\
 -2s_u & .. & -2s_u & -s_u
 \end{bmatrix}
 $ $\in \mathbb{R}^{n_u \times n_u}$,
 
 $s_u$ is the time scaling factor that determines the exponential decay rate, $n_u$ is the number of terms of Laguerre polynomials, and the initial condition is $X(0) =\sqrt{2s_u}[1, 1, ... ,1]^T$ $\in \mathbb{R}^{n_u}$. The accuracy of the approximation increases as the number of terms increases. This approach provides a simple and efficient method to mathematically model the control trajectory with minimum prior information. Also it simplifies the solutions and enable us to tune the predictive control system via only its two parameters (i.e., $s_u$ and $n_u$). This is unlike the classic design of the MPC which is based on Taylor series expansion that provides  non-parametric description for the MPC control trajectory. 

% 
 Considering the moving time window from $t_i$ to $t_i$ + $T_p$, and the time variable within this window is $\iota$, the derivative of the control signal, $\dot{u}_{mpc}(\iota)$, can be described by this set of functions as
 \begin{equation}
 \dot{u}_{mpc}(\iota) = X(\iota)^T \eta,
 \label{eq:umpc_lag}
 \end{equation}
 where $\eta = [c_{u_1}, c_{u_1}, ..., c_{u_{n_u}}]^T$ is a coefficient vector, which will be designed later.
 
 \subsection{Predicted plant response}
 
 The predicted future state vector at time $\iota$ is given as
 \begin{equation}
 x_a(t_i + \iota|t_i) = e^{A_a \iota} x_a(\iota) + \Phi_{mpc}(\iota)^T \eta,
 \label{eq:x_pre}
 \end{equation}
 where $\Phi_{mpc}(\iota)^T = \int_{0}^{\iota} e^{A_a (\iota - \gamma)} B X(\gamma)^T d\gamma$.
 From the prediction of the state variable, the predicted output at time $\iota$
 is
 \begin{equation}
 q_i(t_i + \iota|t_i) = C_a e^{A \iota} x_a(t_i) + C_a \Phi_{mpc}(\iota)^T \eta.
 \label{eq:q_pre}
 \end{equation}
 
 Computation of $\Phi_{mpc}(\iota)$ can be obtained in a recursive solution in terms of $\iota$ = 0, $h$, 2$h$, ..., $T_p$, by
 \begin{equation}
 \Phi_{mpc}(k h)^T = e^{A_a h} \Phi_{mpc}((k-1) h)^T + \Phi_{mpc}(h)^T e^{(k-1)A_u^T h}.
 \label{eq:phi_rec}
 \end{equation}
 
 \subsection{Optimal control strategy}
 
The MPC design is based on the solution of the so-called Finite Horizon Optimal Control Problem which consists of minimizing a suitably defined cost function with respect to the control sequence. The cost function at time $t_i$ is
\begin{align}
	J_{mpc} = \int_0^{T_p} (q_r(t_i) - q(t_i+\iota|t_i))^T Q_{mpc} (q_r(t_i) - q(t_i+\iota|t_i)) +  \dot{u}_{mpc}^T(\iota) R_{mpc} \dot{u}_{mpc}(\iota) d\iota,
	\label{eq:obj_fun}
\end{align}
where $Q_{mpc}$ and  $R_{mpc}$ are weighting matrices that must be positive semi-definite and positive definite, respectively, to ensure the stability of the outer loop \cite{mayne2000constrained}. The optimal control $\dot{u}_{mpc}(\iota)$ can be calculated by minimizing this cost function, $J_{mpc}$, which is the optimal control within the moving window.

By substituting the prediction of the state variable $x_a(t_i + \iota|t_i)$ from (\ref{eq:x_pre}) into (\ref{eq:obj_fun}), the cost function becomes function of $\eta$ as 
\begin{align}
J_{mpc} &= (\eta + \Omega_{mpc}^{-1} \Psi_{mpc} x_a(t_i))^T \Omega_{mpc} (\eta + \Omega_{mpc}^{-1} \Psi_{mpc} x_a(t_i)) \\  
&+ x_a(t_i)^T \int_0^{T_p} e^{A^T \iota} Q_{mpc} e^{A \iota} -  x_a(t_i)^T \Psi_{mpc}^T \Omega_{mpc}^{-1} \Psi_{mpc} x_a (t_i). 
\label{eq:obj_fun2}
\end{align}

Then, by minimizing this cost function in terms of $\eta$, the optimal $\eta$ is 
\begin{equation}
	\eta = - \Omega_{mpc}^{-1} \Psi_{mpc} x_a(t_i), 
	\label{eq:eta_opt}
\end{equation}
where $\Omega_{mpc} = \int_{0}^{T_p} \Phi_{mpc}(\iota) Q_{mpc} \Phi_{mpc}(\iota)^T d \iota + R_{mpc}$, and $\Psi_{mpc} = \int_{0}^{T_p} \Phi_{mpc}(\iota) Q_{mpc} e^{A_a \iota} d \iota$. Thus, the optimal control signal can be calculated, from (\ref{eq:umpc_lag}), in the window from $0\leq  \iota \leq T_p$.

It is difficult to obtain the analytical solutions for these integral expressions, $\Omega_{mpc}$ and $\Psi_{mpc}$. However, these matrices are computed over a given prediction horizon $T_p$. Thus, the integral expressions can be evaluated off-line using a numerical approximation as
\begin{equation}
\Omega_{mpc} = \sum_{k=0}^{T_p} \Phi_{mpc}(k h) Q_{mpc} \Phi_{mpc}(k h)^T h + R_{mpc},
\label{eq:omg_opt}
\end{equation}
\begin{equation}
\Psi_{mpc} = \sum_{k=0}^{T_p} \Phi_{mpc}(k h) Q_{mpc} e^{A_a k h} h.
\label{eq:psi_opt}
\end{equation}

By applying the principle of receding horizon control (i.e., the control action will use only the derivative of the future control signal at $\iota$ = $0$), one can get the derivative of the optimal control as following:
\begin{equation}
	\dot{u}_{mpc}(t) = - X(0)^T \Omega_{mpc}^{-1} \Psi_{mpc} x_a(t),
	\label{eq:umpc_lag2}
\end{equation}

 \subsection{Constrained control}
 
The next step is to formulate the constraints as part of the design requirements, and relate them to the original model predictive control problem. Since the predictive control problem is formulated and solved in the framework of receding horizon control, the constraints are taken into consideration frame-by-frame for each moving horizon window. This gives us the means to solve the constrained control problem numerically. 

The considered constraints, in this work, are that of the robot actuators ($u^{min}\leq  u \leq u^{max}$). Thus, firstly, we have to relate them to the optimized control trajectory of the MPC (i.e., $u_{mpc}^{min}\leq  u_{mpc} \leq u_{mpc}^{max}$) as following: 

The input torque from the controller and applied to the robot, $\tau$, can be calculated from
\begin{equation}
\tau =  \tau_{mpc} + \hat{\tau}^{dis} 
\label{eq:cnst_tau1}
\end{equation}
where $\tau_{mpc}$ is the torque generated from the MPC controller and it can be calculated from
\begin{equation}
 \tau_{mpc} = M_n \ddot{q}^{des} = M_n u_{mpc}. 
\label{eq:cnst_tau2}
\end{equation}
Thus, one can build the following constraints on $\tau_{mpc}$ as
\begin{equation}
\tau^{min} - \hat{\tau}^{dis} \leq \tau_{mpc} \leq \tau^{max} - \hat{\tau}^{dis}.
\label{eq:cnst_tau3}
\end{equation}

%The maximum allowable input torques for the robot can stated as
%
%\begin{equation}
%\tau^{max} = [\tau_x^{max} \  \tau_y^{max} \ \tau_z^{max} \ \tau_{\psi}^{max} \ \tau_{\theta}^{max} \ \tau_{\phi}^{max} \ \tau_{m_1}^{max} \ \tau_{m_2}^{max} \ ]^T.
%\label{eq:cnst_tau4}
%\end{equation}
%\begin{thisnote}
The generalized input forces, $\tau$, can be related to the actuators' inputs via (\ref{thrust_sum} - \ref{Ta3} and \ref{eq:sigmad}) as

\begin{equation}
\tau = \begin{bmatrix} 
\tau_x \\  \tau_y \\ \tau_z \\ \tau_{\psi} \\ \tau_{\theta} \\ \tau_{\phi} \\ \tau_{m_1} \\ \tau_{m_2} 
\end{bmatrix} 
= 
\begin{bmatrix} 
\tau_z (\theta C_{\psi} + \phi S_{\psi}) \\
\tau_z (\theta S_{\psi} - \phi C_{\psi}) \\
F_1 + F_2 + F_3 + F_4 \\
-\gamma_1 F_1 + \gamma_2 F_2 -\gamma_3 F_3 + \gamma_4 F_4 \\
d_q (F_3 - F_1) \\
d_q (F_4 - F_2) \\
\tau_{m_1}\\
\tau_{m_2}\\
\end{bmatrix}.
\label{eq:cnst_tauf}
\end{equation}
By reformulating the 3$^{rd}$ to the 6$^{th}$ element in (\ref{eq:cnst_tauf}), one can get the thrusters' inputs as following
\begin{equation}
\begin{bmatrix} 
F_1 \\  F_2 \\ F_3 \\ F_4 \\
\end{bmatrix} 
= 
\begin{bmatrix} 
\frac{\tau_z}{4} + \frac{\tau_{\psi}}{4 \gamma_1} - \frac{\tau_{\theta}}{2 d_q} \\
\frac{\tau_z}{4} - \frac{\tau_{\psi}}{4 \gamma_2} + \frac{\tau_{\phi}}{2 d_q} \\
\frac{\tau_z}{4} + \frac{\tau_{\psi}}{4 \gamma_3} + \frac{\tau_{\theta}}{2 d_q} \\
\frac{\tau_z}{4} - \frac{\tau_{\psi}}{4 \gamma_4} - \frac{\tau_{\phi}}{2 d_q} \\
\end{bmatrix}.
\label{eq:cnst_tauf2}
\end{equation}
To constrain the thrusters' input to be $F^{min} \leq F_i \leq F^{max}$, relation (\ref{eq:cnst_tauf2}) can be utilized to get the following constraints on the robot's inputs $\tau_z$, $\tau_{\psi}$, $\tau_{\theta}$, and $\tau_{\phi}$.

\underline{\textbf{Constraints for} $\tau_z$}:

To calculate the required constraints on $\tau_z$, each row in (\ref{eq:cnst_tauf2}) is solved to satisfy the constrain $F_i = [F^{min}, F^{max}]$. Thus, there are four constraints on $\tau_z$. The minimum values of the constraints are given by  
\begin{equation}
\begin{bmatrix} 
\tau_z^{min^1} \\  \tau_z^{min^2} \\ \tau_z^{min^3} \\ \tau_z^{min^4}\\
\end{bmatrix} 
= 
\begin{bmatrix} 
4 F^{min} - \frac{\tau_{\psi}}{\gamma_1} +  \frac{2\tau_{\theta}}{d_q}\\
4 F^{min} + \frac{\tau_{\psi}}{\gamma_2} -  \frac{2\tau_{\phi}}{d_q} \\
4 F^{min} - \frac{\tau_{\psi}}{\gamma_3} -  \frac{2\tau_{\theta}}{d_q} \\
4 F^{min} + \frac{\tau_{\psi}}{\gamma_4} +  \frac{2\tau_{\phi}}{d_q} \\
\end{bmatrix},
\label{eq:cnst_Tz}
\end{equation}
where $\tau_z^{min^i}$ is the lower limit of the $\tau_z$ constraint obtained from the constraint of $F_i$.

The maximum values of the constraints are given by
\begin{equation}
\begin{bmatrix} 
\tau_z^{max^1} \\  \tau_z^{max^2} \\ \tau_z^{max^3} \\ \tau_z^{max^4}\\
\end{bmatrix} 
= 
\begin{bmatrix} 
4 F^{max} - \frac{\tau_{\psi}}{\gamma_1} +  \frac{2\tau_{\theta}}{d_q}\\
4 F^{max} + \frac{\tau_{\psi}}{\gamma_2} -  \frac{2\tau_{\phi}}{d_q} \\
4 F^{max} - \frac{\tau_{\psi}}{\gamma_3} -  \frac{2\tau_{\theta}}{d_q} \\
4 F^{max} + \frac{\tau_{\psi}}{\gamma_4} +  \frac{2\tau_{\phi}}{d_q} \\
\end{bmatrix}.
\label{eq:cnst_Tz2}
\end{equation}
While $\tau_z^{min}$ can be calculated from
\begin{equation}
\tau_z^{min}= \max(\tau_z^{min^1}, \tau_z^{min^2}, \tau_z^{min^3}, \tau_z^{min^4}),
\end{equation}
and $\tau_z^{max}$ can be calculated from
\begin{equation}
\tau_z^{max}= \min(\tau_z^{max^1}, \tau_z^{max^2}, \tau_z^{max^3}, \tau_z^{max^4}).
\end{equation}
The torques, $\tau_{\psi}$, $\tau_{\theta}$ and $\tau_{\phi}$, in the right side of (\ref{eq:cnst_Tz} and \ref{eq:cnst_Tz2}) are substituted by their values from last time step (i.e., $\tau_{\psi} (t - \delta t)$, $\tau_{\theta}(t - \delta t)$ and $\tau_{\phi}(t - \delta t)$) or by their predicted values (i.e., $\tau_{\psi} (t - \delta t) + \Delta \tau_{\psi} (t - \delta t)$, $\tau_{\theta}(t - \delta t) + \Delta \tau_{\theta} (t - \delta t)$, and $\tau_{\phi}(t - \delta t)+ \Delta \tau_{\phi} (t - \delta t)$). Where $\Delta \tau_{.} (t - \delta t) = \tau_{.} (t - \delta t) - \tau_{.} (t - 2 \delta t)$. Both of these two cases are tested.

Similarly, the constraints for $\tau_{\psi}$, $\tau_{\theta}$, and $\tau_{\phi}$ are calculated as:
 
\underline{\textbf{Constraints for} $\tau_{\psi}$}:
  
\begin{equation}
\begin{bmatrix} 
\tau_{\psi}^{min^1} \\  \tau_{\psi}^{min^2} \\ \tau_{\psi}^{min^3} \\ \tau_{\psi}^{min^4}\\
\end{bmatrix} 
= 
\begin{bmatrix} 
\gamma_1 (4F^{min} - \tau_z + \frac{2 \tau_{\theta}}{d_q})\\
\gamma_2 (-4 F^{max} + \tau_z + \frac{2 \tau_{\phi}}{d_q})\\
\gamma_3 (4 F^{min} - \tau_z - \frac{2 \tau_{\theta}}{d_q})\\
\gamma_4 (-4 F^{max} + \tau_z - \frac{2 \tau_{\phi}}{d_q})\\
\end{bmatrix}.
\label{eq:cnst_Tep}
\end{equation}
The maximum values of the constraints are given by
\begin{equation}
\begin{bmatrix} 
\tau_{\psi}^{max^1} \\  \tau_{\psi}^{max^2} \\ \tau_{\psi}^{max^3} \\ \tau_{\psi}^{max^4}\\
\end{bmatrix} 
= 
\begin{bmatrix} 
\gamma_1 (4F^{max} - \tau_z + \frac{2 \tau_{\theta}}{d_q})\\
\gamma_2 (-4 F^{min} + \tau_z + \frac{2 \tau_{\phi}}{d_q})\\
\gamma_3 (4 F^{max} - \tau_z - \frac{2 \tau_{\theta}}{d_q})\\
\gamma_4 (-4 F^{min} + \tau_z - \frac{2 \tau_{\phi}}{d_q})\\
\end{bmatrix}.
\label{eq:cnst_Tep2}
\end{equation}
While $\tau_{\psi}^{min}$ can be calculated from
\begin{equation}
\tau_{\psi}^{min}= \max(\tau_{\psi}^{min^1}, \tau_{\psi}^{min^2}, \tau_{\psi}^{min^3}, \tau_{\psi}^{min^4}),
\end{equation}
and $\tau_{\psi}^{max}$ can be calculated from
\begin{equation}
\tau_{\psi}^{max}= \min(\tau_{\psi}^{max^1}, \tau_{\psi}^{max^2}, \tau_{\psi}^{max^3}, \tau_{\psi}^{max^4}).
\end{equation}

\underline{\textbf{Constraints for} $\tau_{\theta}$}:

\begin{equation}
\begin{bmatrix} 
\tau_{\theta}^{min^1} \\ \tau_{\theta}^{min^3}\\
\end{bmatrix} 
= 
\begin{bmatrix} 
2 d_q (- F^{max} + \frac{\tau_z}{4} + \frac{\tau_{\psi}}{4 \gamma_1})\\
2 d_q (F^{min} - \frac{\tau_z}{4} - \frac{\tau_{\psi}}{4 \gamma_3})\\
\end{bmatrix}.
\label{eq:cnst_Tth}
\end{equation}
The maximum values of the constraints are given by
\begin{equation}
\begin{bmatrix} 
\tau_{\theta}^{max^1} \\  \tau_{\theta}^{max^3}\\
\end{bmatrix} 
= 
\begin{bmatrix} 
2 d_q (- F^{min} + \frac{\tau_z}{4} + \frac{\tau_{\psi}}{4 \gamma_1})\\
2 d_q (F^{max} - \frac{\tau_z}{4} - \frac{\tau_{\psi}}{4 \gamma_3})\\
\end{bmatrix}.
\label{eq:cnst_Tth2}
\end{equation}
While $\tau_{\theta}^{min}$ can be calculated from
\begin{equation}
\tau_{\theta}^{min}= \max(\tau_{\theta}^{min^1}, \tau_{\theta}^{min^3}),
\end{equation}
and $\tau_{\theta}^{max}$ can be calculated from
\begin{equation}
\tau_{\theta}^{max}= \min(\tau_{\theta}^{max^1}, \tau_{\theta}^{max^3}).
\end{equation}

\underline{\textbf{Constraints for} $\tau_{\phi}$}:

\begin{equation}
\begin{bmatrix} 
\tau_{\phi}^{min^2} \\ \tau_{\phi}^{min^4}\\
\end{bmatrix} 
= 
\begin{bmatrix} 
2 d_q (F^{min} - \frac{\tau_z}{4} + \frac{\tau_{\psi}}{4 \gamma_2})\\
2 d_q (-F^{max} + \frac{\tau_z}{4} - \frac{\tau_{\psi}}{4 \gamma_4})\\
\end{bmatrix}.
\label{eq:cnst_Tph}
\end{equation}
The maximum values of the constraints are given by
\begin{equation}
\begin{bmatrix} 
\tau_{\phi}^{max^1} \\  \tau_{\phi}^{max^3}\\
\end{bmatrix} 
= 
\begin{bmatrix} 
2 d_q (F^{max} - \frac{\tau_z}{4} + \frac{\tau_{\psi}}{4 \gamma_2})\\
2 d_q (-F^{min} + \frac{\tau_z}{4} - \frac{\tau_{\psi}}{4 \gamma_4})\\
\end{bmatrix}.
\label{eq:cnst_Tph2}
\end{equation}
While $\tau_{\phi}^{min}$ can be calculated from
\begin{equation}
\tau_{\phi}^{min}= \max(\tau_{\phi}^{min^2}, \tau_{\phi}^{min^4}),
\end{equation}
and $\tau_{\phi}^{max}$ can be calculated from
\begin{equation}
\tau_{\phi}^{max}= \min(\tau_{\phi}^{max^2}, \tau_{\phi}^{max^4}).
\end{equation}

\underline{\textbf{Constraints for} $\tau_x$ and $\tau_y$}:

From the 1$^{st}$ and 2$^{nd}$ elements in (\ref{eq:cnst_tauf}), one can get the constraints for $\tau_x$ and $\tau_y$ as:

If $(\theta C_{\psi} + \phi S_{\psi}) > 0$, then
\begin{gather}
\tau_x^{min} =  (\theta C_{\psi} + \phi S_{\psi}) \tau_z^{min}, \\
\tau_x^{max} =  (\theta C_{\psi} + \phi S_{\psi}) \tau_z^{max}.
\end{gather}
If $(\theta C_{\psi} + \phi S_{\psi}) < 0$, then
\begin{gather}
\tau_x^{min} =  (\theta C_{\psi} + \phi S_{\psi}) \tau_z^{max}, \\
\tau_x^{max} =  (\theta C_{\psi} + \phi S_{\psi}) \tau_z^{min}.
\end{gather}

If $(\theta S_{\psi} - \phi C_{\psi}) > 0$, then
\begin{gather}
\tau_y^{min} =  (\theta S_{\psi} - \phi C_{\psi}) \tau_z^{min}, \\
\tau_y^{max} =  (\theta S_{\psi} - \phi C_{\psi}) \tau_z^{max}.
\end{gather}

If $(\theta S_{\psi} - \phi C_{\psi}) < 0$, then
\begin{gather}
\tau_y^{min} =  (\theta S_{\psi} - \phi C_{\psi}) \tau_z^{max}, \\
\tau_y^{max} =  (\theta S_{\psi} - \phi C_{\psi})\tau_z^{min}.
\end{gather}

In the case that the coefficients, $(\theta C_{\psi} + \phi S_{\psi})$ and $(\theta S_{\psi} - \phi C_{\psi})$, are very small, the constraints on the $\tau_x$ and $\tau_y$ are released to keep a minimum distance between the upper and lower limits of $\tau_x$ and $\tau_y$ as following:

If $\tau_x^{max} \leq \tau_x^{s}$, then $\tau_x^{max} = \tau_x^{s}$. If $\tau_x^{min} \leq -\tau_x^{s}$, then $\tau_x^{min} = -\tau_x^{s}$. If $\tau_y^{max} \leq \tau_y^{s}$, then $\tau_y^{max} = \tau_y^{s}$. If $\tau_y^{min} \leq -\tau_y^{s}$, then $\tau_y^{min} = -\tau_y^{s}$. Where $\tau_x^{s}$ and $\tau_y^{s}$ are constants.

\underline{\textbf{Constraints for} $\tau_{m_1}$ and $\tau_{m_2}$ }:
These constraints can be obtained directly from the joints motors' data sheet which they are the limits on the joints motors' torques.

After calculating the limits for the constraints of the input torques, the next step is to calculate the limits for the $u_{mpc}$ as

\begin{equation}
\frac{\tau^{min} - \hat{\tau}^{dis}}{M_n} \leq u_{mpc} \leq \frac{\tau^{max} - \hat{\tau}^{dis}}{M_n}, 
\label{eq:cnst_tau6}
\end{equation}
This means that 
\begin{equation}
u_{mpc}^{min} = \frac{\tau^{min} - \hat{\tau}^{dis}}{M_n},
\label{eq:cnst_tau7}
\end{equation}

\begin{equation}
u_{mpc}^{max} = \frac{\tau^{max} - \hat{\tau}^{dis}}{M_n}.
\label{eq:cnst_tau8}
\end{equation}
Since these constraints are time varying, they will be calculated at the start of each time window ($T_p$) then they are hold (i.e., zero order hold) for the reset period of this window.
%\end{thisnote}
Now we will illustrate how the MPC will constrain the $u_{mpc}$.

Let us assume that $\delta t$ is the sampling interval for implementation, the first sample of the control signal at the optimization window, is calculated as
\begin{equation}
u_{mpc} (t_i) = u_{mpc} (t_i - \delta t) +  X(0)^T \eta \delta t,
\label{eq:u_mpc2}
\end{equation} 
where $u_{mpc}(t_i-\delta t)$ is the previous information of the control signal which is shifted backward by $\delta t$.

Thus, at the first sample time of the window,  the control signal constraints are
\begin{equation}
u_{mpc}^{min} - u_{mpc}(t_i - \delta t)\leq X(0)^T \eta \delta t \leq u_{mpc}^{max} - u_{mpc}(t_i-\delta t).
\label{eq:u_const1}
\end{equation} 
However, at the arbitrary time $\iota_i$, the control signal is
\begin{align}
u_{mpc} (\iota_i) &= u_{mpc} (t_i) + \int_{0}^{\iota_i} \dot{u}_{mpc}(\gamma) d \gamma\\ \nonumber
 &= u_{mpc} (t_i) + (X(\iota_i) - X(0))^T A_u^{-T} \eta.
\label{eq:u_mpc3}
\end{align} 
With the information of $u(t_i - \delta t)$, the future control signal at time $\iota_i$ is presented as

\begin{equation}
u_{mpc} (\iota_i) = u_{mpc} (t_i - \delta t) + (X(0)^T \delta t + X(\iota_i)^T A_u^{-T} - X(0) A_u^{-T}) \eta.
\label{eq:u_mpc4}
\end{equation} 
Thus, the inequality constraints of the control signal are expressed as
\begin{equation}
u_{mpc}^{min} - u_{mpc}(t_i-\delta t)\leq C_u \eta \leq u_{mpc}^{max} - u_{mpc}(t_i-\delta t),
\label{eq:u_const}
\end{equation} 
where $C_u = X(0)^T \delta t + X(\iota_i)^T A_u^{-T} - X(0)^T A_u^{-T}$.

These constraints can be reformulated as linear inequalities as following
\begin{equation}
M_{mpc} \eta \leq \gamma_{mpc},
\label{eq:u_const2}
\end{equation} 
where
\begin{equation}
M_{mpc} = \begin{bmatrix}   
X(0)^T \delta t + X(\iota_i)^T A_u^{-T} - X(0)^T A_u^{-T}\\ -(X(0)^T \delta t + X(\iota_i)^T A_u^{-T} - X(0)^T A_u^{-T})        
\end{bmatrix},
 \end{equation} 
 and
 \begin{equation}
\gamma_{mpc} = \begin{bmatrix}  
u_{mpc}^{max} - u_{mpc}(t_i-\delta t)  \\ - u_{mpc}^{min} + u_{mpc}(t_i-\delta t) \end{bmatrix}.
\end{equation}  
Since the objective function (\ref{eq:obj_fun2}) is quadratic, and the constraints are linear inequalities, the problem of finding an optimal predictive control becomes one of finding an optimal solution to a standard quadratic programming problem. These inequality constraints consist of active constraints and inactive
constraints. An inequality $M_{mpc} \eta \leq \gamma_{mpc}$ is said to be active if $M_{mpc} \eta = \gamma_{mpc}$ and inactive if $M_{mpc} \eta < \gamma_{mpc}$.

A simple and efficient algorithm, called Hildreth's quadratic programming procedure \cite{wismer1978introduction}, is proposed for solving this problem.  In this method, to reduce the computational load, the constraints that are not active is identified systematically, then they are eliminated in the solution. The active constraints are equality constraints, so one can rely on the Lagrange multipliers, $\Lambda$, to solve this optimization problem (Quadratic objective function with equality constraints). This method will lead to very simple programming procedures for finding optimal solutions of constrained minimization problems. This algorithm is based on an element-by-element search, therefore, it does not require any matrix inversion. 

In this method, the $i^{th}$ Lagrange multiplier at iteration $k+1$ is calculated from  

\begin{equation}
\Lambda_i^{k+1} = \max(0,W_i^{k+1}),
\label{eq:lamda}
\end{equation}
where
\begin{equation}
W_i^{k+1} = -\frac{1}{h_{ii}}(e_i + \sum_{j=1}^{i-1} h_{ij} \Lambda_j^{k+1} + \sum_{j=i+1}^{n} h_{ij} \Lambda_j^{k}),
\label{eq:WW}
\end{equation}
$h_{ij}$ represents the $ij^{th}$ element of the matrix $H_{mpc} = M_{mpc} \Omega_{mpc}^{-1} M_{mpc}^T$, and $e_i$ is the $i^{th}$ element of the vector $E_{mpc} = \gamma_{mpc} + M_{mpc} \Omega_{mpc}^{-1} \Psi_{mpc} x_a$. 

The iteration will be terminated when the iterative counter reaches its maximum value, $m_{max}$, at which the $\Lambda$ converges to its optimal value, $\Lambda^*$, which contains zeros for inactive constraints and the positive components corresponding to the active constraints. Then, the optimal $\eta$ can be calculated from
\begin{equation}
\eta^* = - \Omega_{mpc}^{-1} (\Psi_{mpc} + M_{mpc}^T \Lambda^*),
\label{eq:eta}
\end{equation}
and thus the optimal control signal can be obtained from
\begin{equation}
u_{mpc}^* (t) = \int_{0}^{t} \dot{u}_{mpc}^*(\iota) d\iota.
\label{eq:umpc_lag3}
\end{equation} 
with 
\begin{equation}
\dot{u}_{mpc}^*(\iota) = X(\iota)^T \eta^*.
\label{eq:umpc_lag4}
\end{equation}
Summery of the MPC technique is presented as algorithm \ref{alg:mpc}.

\begin{algorithm}
%	\SetAlgoLined
	\caption{MPC algorithm}
	\label{alg:mpc}
	\begin{algorithmic}[1]
		\State time $t$ = $t_i$
		\While{($t \leq t_f$)}
		\For{$t = t_i:\delta t:T_p$}
		\State Get the current state $x_a(t)$
	    \State Solve the Optimal Control Problem numerically by minimizing the cost function $J_{mpc}$ subjected to the constraints (\ref{eq:u_const2})
	    \State Find the optimal control sequence $u_{mpc}^*(t_i)$ \ldots $u_{mpc}^*(\iota)$ \ldots $u_{mpc}^*(T_p)$
	    \State Apply only $u_{mpc}^*(t_i)$ 
		\EndFor \Comment{ At time $t = t_i + \delta t$: Get new measurements, repeat the optimization, and so on.}
		\EndWhile \Comment{ Repeat the procedure in the next prediction window of length $T_p$ }
	\end{algorithmic}
\end{algorithm} 

%Stability issues of the MPC algorithm was discussed in \cite{wang2009model, anderson1971linear}. One of the techniques that is utilized to guarantee the stability is to use an exponentially weighted objective function which is given by
%\begin{align}
%J = \int_0^{T_p} e^{-2\alpha \iota}(q_r(t_i) - q(t_i+\iota|t_i))^T Q_{mpc} (q_r(t_i) - q(t_i+\iota|t_i)) +  e^{-2\alpha \iota} \dot{u}_{mpc}^T(\iota) R_{mpc} \dot{u}_{mpc}(\iota) d\iota
%\label{eq:obj_fun_expw}
%\end{align}
%where $\alpha$ is the weighting constant. This cost function will lead to the following state equation
%\begin{equation}
%\dot{x}_a(t_i + \iota|t_i) = (A_a - \alpha I) x(t_i + \iota|t_i) + B_a \dot{u}_{mpc}(\iota)
%\label{eq:x_pre_alp}
%\end{equation}
%i.e the system matrix becomes $(A_a - \alpha I)$, and it can be designed to make sure it is stable with all eigen values on the left-half of the complex plane. To guarantee exponential decay of the state variable  within the optimization window, a simple modification of the weight matrix $Q_{mpc}$ is proposed as $Q_{\alpha} = Q_{mpc} + 2 \alpha P_{mpc}$, where $P_{mpc}$ is the solution of the following Riccati equation

%\begin{equation}
%P_{mpc} (A_a-\alpha I) + (A_a-\alpha I)^T P_{mpc} - P_{mpc} B_a R_{mpc}^{-1} B_a^T P_{mpc} + Q_{\alpha} = 0
%\label{eq:RIC_equ}
%\end{equation}  
 \subsection{MPC tuning guidelines}
 The design variables in the continuous time model predictive control algorithm presented above are \cite{wang2001continuous}:
 \begin{itemize}
 	\item Weighting matrices, $Q_{mpc}$ and $R_{mpc}$: The smaller elements in $R_{mpc}$ and larger elements of $Q_{mpc}$ corresponds to faster closed-loop response speed.
 	
 	 \item Pole location of the Laguerre model for the future control signal, $s_u$: is a tuning parameter for the closed-loop response speed. Larger p results in larger changes in the future control signal in the initial period, hence faster closed-loop response speed.
 	 \item Number of terms used in the Laguerre model to capture the control signal, $n_u$: As $n_u$ increases, the degree of freedom in describing the control trajectory increases. The control signal tends to be more aggressive when $n_u$ increases thus faster closed-loop response speed.
 	 
 	 \item Prediction horizon $T_p$: For stable system, the prediction horizon is recommended to be chosen approximately equal to the open loop process settling time. For unstable and integrating processes, which as in our case, $T_p$ is recommended to be chosen as a parameter of $s_u$ approximately equal to ($\frac{10}{s_u}$). 
 	 
 \end{itemize}
Fig. \ref{fig:detail_mpc_dob} shows the complete block diagram of the proposed control system. As it is stated before, the position, the manipulator joints' angles, and the yaw angle are usually the controlled variables, while pitch and roll angles are used as intermediate control inputs for horizontal positions control. Therefore, the proposed control system consists from two DOb-based controllers by dividing $q$ into two parts; one for $\zeta=[x \ y \ z \ \psi \ \theta_1 \ \theta_2]^T$ (with $MPC_{\zeta}$, $M_{n_a}$, $M_{nv_1}$, $P_{v_1}$, $Q_{v_1}$, and $Q_{a}$) and the other for $\sigma_b = [\theta \ \phi]^T$ (with $MPC_{\sigma}$, $M_{nv_2}$, $P_{v_2}$, and $Q_{v_2}$). The desired trajectories for the end-effector's position and orientation ($p_{e,r}$ and $\Phi_{e,r}$) are fed to the inverse kinematics algorithm together with $\sigma_{b,r}(t)$ such that the desired quadrotor/joint space trajectories $\zeta_r(t)$ are obtained. After that, the controller block receives the desired trajectories and the feedback signals from the system and then provides the control signal, $\tau$. The desired values $\sigma_{b,r}$ for the intermediate controller are obtained from the output of position controller, $\tau_{\zeta}$, through (\ref{eq:sigmad})

The output of the two controllers, $\tau_{\zeta}$ and $\tau_{\sigma}$, are mixed to generate the final control vector $\tau$ which is then converted to the forces/torques applied to quadrotor/manipulator via the relation (\ref{eq:ufinal})

% =======================================
\begin{figure}[!h]
	\centering
	\includegraphics[width=1\columnwidth]{detail_mpc_dob}
	\caption{Block diagram of the detailed MPC-DOb control system for the quadrotor manipulation system}
	\label{fig:detail_mpc_dob}
\end{figure}
%==========================================================

\begin{remark}
	It is better to make the response of the $\sigma$ controller faster than that of the quadrotor position controller such that it can track the changes in the position controller \cite{hua2013introduction, isidori2012robust}. This can be achieved by the tuning parameters of both DOb and MPC.
\end{remark}  

\subsection{Simulation Results} \label{se:sim}

In this section the previously proposed control strategy is applied in simulation MATLAB/SIMULINK program to the model of the considered aerial manipulation robot. The simulation environments similar to that in section \ref{se:sim_dob_envirnemnt} is used here. Parameters of the MPC controller are given in Table \ref{tab:DOb_par}.
%============================================
\begin{table}[!h]
	\caption{MPC-DOb controller parameters}
	\label{tab:DOb_par}
	\begin{center}
		\setlength{\tabcolsep}{10pt}
		\begin{tabular}{|c|c|}
			\hline
			Parameter & Value \\
			\hline
			$Q_{mpc_{\zeta}}$ & $C^T C$\\
			\hline
			$R_{mpc_{\zeta}}$	& $I_6$\\
			\hline
			$Q_{mpc_{\sigma}}$ & $2 C^T C$\\
			\hline
			$R_{mpc_{\sigma}}$	& $0.2 I_2$\\
			\hline
			$u^{max}$ & $[6 \ 6 \ 6 \ 6 \ 0.7 \ 0.4]^T$\\
			\hline
			$u^{min}$ & $[0 \ 0 \ 0 \ 0 \ -0.7 \ -0.4]^T$ \\
			\hline
			$s_{u_{\zeta}}$ & $2$\\ 
			\hline
			$s_{u_{\sigma}}$ & $10$\\ 
			\hline
			$n_{u_{\zeta}}$ & $3$\\ 
			\hline
			$n_{u_{\sigma}}$ & $6$\\
			\hline
			$h$ & $0.01$\\
		   \hline
		   $k_{max}$ & $38$\\
		   \hline
		   $\tau_x^{s}$, $\tau_y^{s}$ & 0.5\\
		   \hline
		\end{tabular}
	\end{center}
\end{table}
%==============================================

 The system response in the quadrotor/joint space is presented in Fig. \ref{fig:kin_joint_cform_mpc_results}. Figs. \ref{fig:inv_kin_pp_results} and \ref{fig:3d_traj} show responses of the proposed scheme in the task space (the actual end-effector position and orientation can be found from the forward kinematics). Note that the marker represents the end-effector orientation; Green, Blue, and Red for x-,y-, and z-axis. These results show that the proposed motion control scheme able to track the desired trajectories, and so the control objectives \ref{obj:stab} - \ref{obj:optimal} are achieved. Moreover, the MPC reduces the oscillations that appears at the start of motion by using the PD-DOb method.
 
 Fig. \ref{fig:DOb_effort} shows the control effort, the required thrust forces and manipulator torques which are in the allowable limits. It is noted also from this figure that the control effort becomes lower and has no sharpness than that in the case of using the PD-DOb technique. 
 %============================================
 \begin{figure}[!h]
 	\centering
 	\begin{tabular}{cc}
 		\subfloat[$x$]{\includegraphics[width=0.4\columnwidth]{x_traj_IK_dob}}&
 		\subfloat[$y$]{\includegraphics [width=0.4\columnwidth]{y_traj_IK_mpc_dob}}\\
 		\subfloat[$z$]{\includegraphics [width=0.4\columnwidth]{z_traj_IK_mpc_dob}}&
 		\subfloat[$\psi$]{\includegraphics [width=0.4\columnwidth]{ep_traj_IK_mpc_dob}}\\
 		\subfloat[$\theta_{1}$]{\includegraphics [width=0.4\columnwidth]{th1_traj_IK_mpc_dob}}&
 		\subfloat[$\theta_{2}$]{\includegraphics [width=0.4\columnwidth]{th2_traj_IK_mpc_dob}}
 	\end{tabular}
 	\caption{MPC-DOb results: The actual response in the quadrotor/joint space; a) $x$, b) $y$, c) $z$, d) $\psi$, e) $\theta_{1}$, and f)  $\theta_{2}$}
 	\label{fig:kin_joint_cform_mpc_results}
 \end{figure}
% ==============================================
\begin{figure}[!h]
	\centering
	\begin{tabular}{cc}
		\subfloat[$x_{e}$]{\includegraphics[width=0.4\columnwidth]{xe_traj_IK_mpc_dob}}&
		\subfloat[$y_{e}$]{\includegraphics [width=0.4\columnwidth]{ye_traj_IK_mpc_dob}}\\
		\subfloat[$z_{e}$]{\includegraphics [width=0.4\columnwidth]{ze_traj_IK_mpc_dob}}&
		\subfloat[$\phi_{e}$]{\includegraphics [width=0.4\columnwidth]{phe_traj_IK_mpc_dob}}\\
		\subfloat[$\theta_{e}$]{\includegraphics [width=0.4\columnwidth]{the_traj_IK_mpc_dob}}&
		\subfloat[$\psi_{e}$]{\includegraphics [width=0.4\columnwidth]{epe_traj_IK_mpc_dob}}
	\end{tabular}
	\caption{MPC-DOb results: The actual response of the end-effector pose: a) $x_{e}$, b) $y_{e}$, c) $z_{e}$, d) $\phi_{e}$, e) $\theta_{e}$, and f) $\psi_{e}$}
	\label{fig:inv_kin_pp_results}
\end{figure}
%==============================================

\begin{figure}[!h]
	\centering
\includegraphics[width=0.5\columnwidth]{3D_traj_IK_mpc_dob}
	\caption{MPC-DOb results: 3D task space trajectory}
				\label{fig:3d_traj}	
\end{figure}
%====================================

\begin{figure}[!h]
	\centering
      \includegraphics[width=0.9\columnwidth]{OM_traj_IK_mpc_dob}
	\caption{MPC-DOb results: The required controller efforts}
	\label{fig:DOb_effort}
\end{figure}
%============================================
Table \ref{tab:mpc_vs_pd} presents a comparison study between PD-DOb and MPC-DOb controllers. The first part in this table compares the Root Mean Square Error (RMSE) in the tracking of the end-effector position and orientation. The RMSE of the MPC is slightly lower than that of the PD-DOb. The second part presents the summation of quadrotor thrusters efforts as well as the manipulator torques. This table enlightens the superior performance of the MPC-DOb over the PD-DOb. The using of the MPC leads to a 15 $\%$ reduction in the required thrust effort. 
%============================================
\begin{table}[!h]
	\caption{Comparison study: MPC-DOb vs PD-DOb}
	\label{tab:mpc_vs_pd}
	\begin{center}
		\setlength{\tabcolsep}{10pt}
		\begin{tabular}{|c|c|c|}
			\hline
			RMSE & PD-DOb & MPC-DOb \\
			\hline
			$x_e$ [m] & 0.0390 & 0.0377\\
			\hline
			$y_e$ [m] & 0.0370 & 0.0306\\
			\hline
			$z_e$ [m] & 0.0227 & 0.0031 \\
			\hline
		 	$\psi_e$ [deg] & 0.4469 & 0.0250 \\
			\hline
	    	$\theta_e$ [deg] & 1.0199 & 0.0309 \\
			\hline
		    $\phi_e$ [deg] & 0.2876 & 0.8113 \\
			\hline
		    Control Effort &	 & \\ 
			\hline
			$\sum T$ [N]& 748.3817 & 645.4135 \\
			\hline
			$\sum \tau_{m_1}$ [N.m]& 11.6674 & 11.6460 \\	
			\hline
			$\sum \tau_{m_2}$ [N.m]& 4.6629 & 4.6355 \\	
			\hline
		\end{tabular}
	\end{center}
\end{table}
%==============================================
\clearpage

\section{Robust Force Estimation and Impedance Control} \label{se:ftrls_dob}
 
 In this section, a robust sensorless force estimation and impedance control system is presented to achieve the objectives \ref{obj:stab}, \ref{obj:track}, \ref{obj:force}, and \ref{obj:impd} .

The proposed methodology to satisfy these control objectives is illustrated in Fig. \ref{fig:ftrls_dob_fncblg}. In this control strategy, the system nonlinearities, external disturbance (wind), $\tau_{w}$, and contact force, $\tau_{l}$, are treated as extended disturbances, $\tau^{dis}$, which will be estimated, as $\hat{\tau}^{dis}$, and canceled by the DOb in the inner loop. The system can now be considered as a group of linear SISO subsystems. The output of DOb with system measurements of quadrotor/joint space variables and the derived task space variables are used as the inputs to the Fast Tracking Recursive Least Squares (FTRLS) algorithm to obtain the end-effector contact force $\hat{F}_e$. The task space impedance control is used in the external loop of DOb and its output is transformed to the quadrotor/joint space through a coordination transformation algorithm.
%===================================================
\begin{figure}[!h]
	\centering
	\includegraphics[width=1\columnwidth]{force_dob_fncblg}
	\caption{Functional block diagram of the FTRLS-DOb control system}
	\label{fig:ftrls_dob_fncblg}
\end{figure}
%===================================================
\subsection{Modeling of the Environment Dynamics and the Wind Effect}
 
The dynamical model of the quadrotor-manipulator system (\ref{eq:dyn_gen}) can be rewritten as
\begin{gather}
M(q) \ddot{q} + C(q,\dot{q}) \dot{q} + G(q) + \tau_w + \tau_l=\tau, \nonumber \\
\label{eq:dyn_gen2}
\end{gather}
where $\tau_w $ $ \in \mathbb{R}^{8}$ is the vector of the external wind effect, and $\tau_l $ $ \in \mathbb{R}^{8}$ is the vector of the contact force effect.

The environment dynamics, contact force, $\tau_l$, can be modeled as following.
\begin{equation}
\tau_l = J^T F_e,
\label{eq:Tl}
\end{equation}
where the task space contact force, $F_e$, can be modeled from
% the following algorithm \ref{alg:env_dyn}.
\begin{equation}
F_e= S_c \left(\chi_e - \chi_{e,o} \right)  + D_c \dot{\chi}_e,
\label{eq:fe}
\end{equation}
where the quantity $\chi_{e,o}$ is taken equal to the previous state until the contact occurs. At the contact, $\chi_{e,o}$ is equal to the state at the start of the interaction with the environment. $S_c = diag\{S_{c_1}, S_{c_2}, S_{c_3}, S_{c_4}, S_{c_5}, S_{c_6}\}$ and $D_c = diag\{D_{c_1}, D_{c_2}, D_{c_3}, D_{c_4}, D_{c_5}, D_{c_6}\}$ represent the environment stiffness and the environment damping, respectively. It is to be noted that the algorithm for contact force estimation is always run. If any component of the estimated force exceeds the threshold (0.1 N / 0.01 N.m), contact with the environment is indicated and its consequences are followed. Similarly, if the all components of the estimated force are below the threshold, non-contact condition with environment is indicated and its consequences are followed.

The wind dynamics, $\tau_w$, can be modeled as following \cite{windmodel, hsu2011verifying, andrews2012modeling}:

The wind velocity is determined by 
\begin{equation}
V_{wz} = V_{w_{z_0}} \frac{z}{z_0},
\label{eq:Vwz}
\end{equation}
where $V_{wz}$  is the wind velocity at altitude $z$, $V_{w_{z_0}}$ is the specified wind velocity at altitude $z_0$. 
  
To  simulate  wind  disturbances,  it is worth calculating the wind generalized force, $\tau_{w}$, which influences the platform.  This  force  can  be  determined  by
\begin{equation}
\tau_{w} = 0.61 * A_e V_{wz}^2, 
\label{eq:Fw}
\end{equation}
where $0.61$ is the rate of wind velocity (m/s$^2$) conversion to pressure (N/m$^2$). $A_e$  is the effective area that depends on the quadrotor structure and its orientation which will be presented latter.

This force can be projected on the axes of frame $\Sigma$ as
\begin{equation}
\begin{split}
\tau_{wx} = f_{wx_1} z^2 \sin(\theta) + f_{wx_2} z^2 \cos(\theta), \\
\tau_{wy} = f_{wy_1} z^2 \sin(\phi) + f_{wy_2} z^2 \cos(\phi),
\end{split}
\label{eq:Fwxy}
\end{equation} 
where 
\begin{equation}
f_{wx_1} = 0.61 * A_{e_1} (\frac{V_{w_{z_0}}}{z_0})^2 \cos(\psi_w),
\end{equation} 

\begin{equation}
f_{wx_2} = 0.61 * A_{e_2} (\frac{V_{w_{z_0}}}{z_0})^2 \cos(\psi_w), 
\end{equation}
 
\begin{equation}
f_{wy_1} = 0.61 * A_{e_1} (\frac{V_{w_{z_0}}}{z_0})^2 \sin(\psi_w), 
\end{equation}

\begin{equation}
f_{wy_2} = 0.61 * A_{e_2} (\frac{V_{w_{z_0}}}{z_0})^2 \sin(\psi_w),
\end{equation}

 $\psi_w$ represents the angle of wind direction. Both $A_{e_1}$ and $A_{e_2}$ depend on the quadrotor design parameters and they are given as following:
 
 Let us represent the quadrotor as a cylinder with height, $h_q$, and radius, $r_q$. Thus,
 \begin{equation}
A_{e_1} = \beta_q \pi r_q^2,
 \end{equation} 
 \begin{equation}
  A_{e_2} = \alpha_q \pi r_q h_q,
  \end{equation}
  where $\beta_q$ and $\alpha_q$ are the fill factors of the cylinder areas. 
%===================================================
\subsection{Fast Tracking Recursive Least Squares} \label{sse:sprls}


In this part, a technique is developed which utilizes a Fast Tracking Recursive Least Squares (FTRLS) to estimate the contact force with the aid of the DOb linearization capabilities. The FTRLS algorithm is one of the fast online least squares-based identification methods used for the identification of environments with varying dynamic parameters \cite{hu2014least, wang2015recursive}. To apply FTRLS, the dynamic equations (\ref{eq:dyn_gen2}- \ref{eq:Fwxy}) have to be parametrized (i.e., to be product of measurement data regressor and dynamic parameters) as following.

The system dynamics part, $\tau_{int}=  M(q) \ddot{q} + C(q,\dot{q}) \dot{q} + G(q)$, can be rewritten as the product of data regressor, $Y_i(q,\dot{q},\ddot{q})$, and platform parameters, $h_i$. 
\begin{gather}
h_i = [m_1 \ m_2 \ m \ I_1 \ I_2 \ I_x \ l_0  m_1 \ l_0  m_2 \ l_1  m_1 \ l_1  m_2 \ l_2   m_1 \ l_2  m_2 \ l_0^2  m_1 \ l_0^2  m_2 \ l_1^2 \nonumber \\ m_1 \ l_1^2  m_2 \ l_2^2  m_1 \ l_2^2  m_2   \ l_0  l_1  m1 \ l_0  l_1  m_2 \ l_1  l_2  m_1 \ l_1  l_2  m_2 \ l_0  l_2  m_1 \ l_0 l_2  m_2]^T.
\end{gather} 

The environment dynamics, $\tau_l$, can be reformulated as $Y_l(q,\dot{q},\ddot{q}, \chi_e,\dot{\chi}_e) \ h_l$, where, $Y_l=J^T Y_e$, $Y_e$ is a function of the end effector states, ($\chi_e$,$\dot{\chi}_e$), which can be calculated as 

\begin{equation}
Y_e = \begin{bmatrix}
\chi_{e,e}(1) & \dot{\chi}_{e,e}(1) & O_{1 \times 1} & O_{1 \times 9} \\
O_{1 \times 2} & \chi_{e,e}(2) & \dot{\chi}_{e,e}(2) & O_{1 \times 8} \\
O_{1 \times 4} & \chi_{e,e}(3) & \dot{\chi}_{e,e}(3) & O_{1 \times 6} \\
O_{1 \times 6} & \chi_{e,e}(4) & \dot{\chi}_{e,e}(4) & O_{1 \times 4} \\
O_{1 \times 8} & \chi_{e,e}(5) & \dot{\chi}_{e,e}(5) & O_{1 \times 2} \\
O_{1 \times 9} & \chi_{e,e}(6) & \dot{\chi}_{e,e}(6) & O_{1 \times 1}\\
\end{bmatrix}.
\end{equation} 

$h_l$ is the vector of the environment parameters $S_c$ and $D_c$ and it is given as
\begin{equation}
h_l = [S_{c_1}\ D_{c_1}\ S_{c_2}\ D_{c_2}\ S_{c_3}\ D_{c_3}\ S_{c_4}\ D_{c_4}\ S_{c_5}\ D_{c_5}\ S_{c_6}\ D_{c_6}]^T.
\end{equation}
Finally, the wind effect is formulated as $Y_w(z,\theta,\phi) \ h_w$. $Y_w$ can be calculated as 
\begin{equation}
Y_w = \begin{bmatrix}
z^2 S_{\theta} & z^2 C_{\theta} & 0 & 0 \\
0 & 0 & z^2 S_{\phi} & z^2 C_{\phi}\\
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 \\
\end{bmatrix}.
\end{equation}

$h_w$ is the vector of the wind parameters and it is given as 
\begin{equation}
h_w = [f_{wx_1} \ f_{wx_2}\ f_{wy_1} \ f_{wy_2}]^T.
\end{equation}
Therefore, the total dynamics can be reformulated as
\begin{equation}
\begin{split}
\tau = Y_s \ h_s, \\
Y_s=[Y_i \ Y_l \ Y_w], \\
h_s=[h_i \ h_l \ h_w]^T,
\label{eq:reg_tot}
\end{split}
\end{equation}   
where $Y_s$ $\in \mathbb{R}^{8 \times 40}$ and $h_s$ $\in \mathbb{R}^{40}$ are the data regressor and parameters vector of (\ref{eq:dyn_gen2}), respectively.
The details of $Y_i$ and $Y_l$ are given in Appendix \ref{app:system_Jacobian}.
 
The parameter estimation error is
\begin{equation}
\tilde{h}_s(t) = h_s - \hat{h}_s(t),
\label{eq:SPRLS_eh}
\end{equation}
while the estimation error is
\begin{equation}
\tilde{\tau}(t) = \tau(t) - Y_s(t) \hat{h}_s(t) = Y_s(t) \tilde{h}_s(t).
\label{eq:SPRLS_ey}
\end{equation}

By minimizing a cost function with respect to the parameter estimation error, one can find the time derivative of the estimated parameters vector, $\hat{h}_s$, as following
\begin{equation}
\frac{d}{dt}\hat{h}_s(t)=  R(t) Y_s^{T}(t) \tilde{\tau}(t), 
\label{eq:SPRLS_hd}
\end{equation}
where $R(t)$ is the parameters' covariance matrix, and it can be calculated from
\begin{equation}
\frac{d}{dt}R^{-1}(t) = -\eta_h(t) R^{-1}(t) + Y_s^{T}(t) Y_s(t),
\label{eq:SPRLS_R}
\end{equation}
where $\eta_h$ is the forgetting factor, and it is given as 
\begin{equation}
\eta_h(t) = \eta_h^{min}  + (1-\eta_h^{min}) 2^{(-NINT(\gamma_g \norm{\tilde{\tau}(t)}^2))},
\label{eq:SPRLS_Rg}
\end{equation}
where $\eta_h^{min}$ is a constant representing the minimum forgetting factor, $NINT(.)$ is the round-off operator, and $\gamma_g$ is a design constant. This adaptive formulation of the forgetting factor enables the RLS to track the non-stationary parameters to be estimated.  

Finally, the estimated contact generalized force in the quadrotor/joint space and task space can be calculated from  
\begin{equation}
\begin{split}
\hat{\tau}_l = Y_l \hat{h}_l,\\
\hat{F}_e = Y_e \hat{h}_l.
\end{split}
\label{eq:SPRLS_thl}
\end{equation}
Therefore, unlike the current developed schemes, this technique enables the isolation and the estimation of the end-effector contact force apart from the whole estimated forces in the systems. This estimated force will be utilized in the next section to design an impedance control for the proposed system. Furthermore, for the tele-manipulation, the use of force feedback is essential to assist the human operator in the remote handling of objects. Moreover, it is very critical to get the force feedback to achieve the cooperative grasping among aerial manipulation robots. If the load for the UAVs is heavier than the carrying capacity of a single UAV, multiple UAVs can distribute the load among them and move the object.


\subsection{Impedance Control} \label{sse:impd_ctrl}

The objective of the impedance control is to impose, along each direction of the task space, a desired dynamic relation between the end-effector pose and the force of interaction with the environment (i.e., desired impedance).
The linear impedance control is designed in the task space. This is based on the linearization effect of the designed DOb in the quadrotor/joint space.
The desired acceleration in the task space, $\ddot{\chi}^{des}_e$, can be calculated from
\begin{equation}
\ddot{\chi}^{des}_e = \ddot{\chi}_{e,r} + M_{c,d}^{-1} \left(S_{c,d} (\chi_{e,r} -  \chi_{e}) + D_{c,d} (\dot{\chi}_{e,r} -  \dot{\chi}_{e}) - \hat{F}_e \right),
\label{eq:xe_des}
\end{equation}
where $M_{c,d}$, $S_{c,d}$, and $D_{c,d}$ are constant diagonal positive definite matrices representing the desired inertia, stiffness, and damping, respectively, which determine the desired impedance that the end-effector will apply to the environment.

The control law (\ref{eq:xe_des}) is active during the contact between the end-effector and the environment. Another control is used during the non-contact which is a tracking PD controller and it is given as
\begin{equation}
\ddot{\chi}^{des}_e = \ddot{\chi}_{e,r} +  K_{P,e} (\chi_{e,r} -  \chi_{e}) + K_{D,e} (\dot{\chi}_{e,r} -  \dot{\chi}_{e}),
\label{eq:xe_des2}
\end{equation}
where $K_{P,e}$ and $K_{D,e}$ are constant diagonal positive definite matrices representing the proportional and derivative gains of the task space PD controller. Thereby, if the contact occurs the task space desired accelerations are computed from (\ref{eq:xe_des}) while they are calculated from \ref{eq:xe_des2} if there is no contact.


Fig. \ref{fig:detail_impd_dob} shows the complete block diagram of the proposed control system during contact. The quadrotor position, the manipulator joints' angles and the yaw angle are usually the controlled variables, while pitch and roll angles are used as intermediate control inputs for horizontal positions control. Therefore, the proposed control system consists from two DOb-based controllers by dividing $q$ into two parts; one for $\zeta=[x \ y \ z \ \psi, \theta_1 \ \theta_2]^T$ (with $K_{imp}$, $Q_{a}$, $M_{n_a}$, $M_{nv_1}$, $P_{v_1}$, $Q_{v_1}$) and the other for $\sigma_b = [\theta \ \phi]^T$ (with $K_{\sigma}$, $M_{nv_2}$, $P_{v_2}$, and $Q_{v_2}$). The desired trajectories for the end-effector's position and orientation, $\chi_{e,r}$, their actual values (by using the forward kinematics), and the estimated end-effector force, are fed to the impedance control law, $K_{imp}$ that is described in (\ref{eq:xe_des}). Then, a coordination transformation from task space to quadrotor/joint space is done by using (\ref{eq:qdd_des}) to obtain $\ddot{\zeta}^{des}$. The desired acceleration in the quadrotor/joint space, $\ddot{\zeta}^{des}$, can be calculated by differentiating (\ref{eq:xedot}) with respect to time as
\begin{equation}
\ddot{\zeta}^{des} = J_{\zeta}^{-1} \left(Q_e \ddot{\chi}^{des}_e + \dot{Q}_e \dot{\chi}_{e,r} - \dot{J}_{\zeta} \dot{\zeta} - J_{\sigma} \ddot{\sigma}_b - \dot{J}_{\sigma} \dot{\sigma}_b \right), 
\label{eq:qdd_des}
\end{equation}

The desired acceleration in quadrotor/joint space, $\ddot{\zeta}^{des}$, is then applied to the DOb of the independent coordinates, $\zeta$, to produce $\tau_{\zeta}$. The desired values for the intermediate DOb controller, $\sigma_{b,r}$, are obtained from the output of position controller, $\tau_{\zeta}$, through (\ref{eq:sigmad}).

The external controller of the DOb for $\sigma$, $\tau_{\sigma}$, is used as a proportional controller with velocity feedback, $K_{\sigma}$, as following:
\begin{equation}
\ddot{\sigma}_b^{des} = K_{p_{\sigma}} (\sigma_{b,r} - \sigma_{b}) - K_{d_{\sigma}} \dot{\sigma}_{b}.
\label{eq:K_sig}
\end{equation}
After that, $\ddot{\sigma}^{des}$ is applied to the DOb for $\sigma$ to generate $\tau_{\sigma}$.

However, the response of the $\sigma$ controller must be much faster than that of the quadrotor position controller such that it can track the changes in the position controller. This can be achieved by the tuning parameters of both the DOb and the proportional controller with velocity feedback of $\sigma_b$.  

The output of the two controllers, $\tau_{\zeta}$ and $\tau_{\sigma}$, are combined together to generate the final control vector $\tau$ which is then converted to the forces/torques applied to quadrotor/manipulator through (\ref{eq:ufinal}).

% =======================================
\begin{figure}[!h]
	\centering
	\includegraphics[width=1\textwidth]{detail_impd_dob}
	\caption{Block diagram of the detailed FTRLS-DOb control system for the quadrotor manipulation system}
	\label{fig:detail_impd_dob}
\end{figure}
%==========================================================

\subsection{Simulation Results}

In this section, the previously proposed control strategy is applied in MATLAB/SIMULINK to the model of the considered aerial manipulation robot with the same setup of section \ref{se:sim_dob_envirnemnt}.
 
Parameters of the proposed algorithm are given in Table \ref{tab:ftrls_DOb_par}. The profile of the wind angle, $\psi_w$, is simulated as in Fig. \ref{fig:wind_angle}. To emulate a real scenario, the value $V_{w_{z_0}}$ is chosen to has two parts; the first one is constant and the second part is random variable to simulate the gust effect (sudden and random changes in the wind speed), see Fig. \ref{fig:wind_speed}.
 
The aim of considered case study is to perform tracking of the desired 6-DOF end-effector trajectories (i.e., circular helix for the position and Quintic trajectories for the orientation) while an external force of 1.6 N acts along the z-axis of the end-effector, $z_e$, for $z_e \leq 10$ cm (i.e., the contact occurs during period from 50 s to 60 s). This scenario simulates, for instance, the case of the manipulator in contact with a soft environment. Thereby, the manipulator end-effector is chosen to be rigid. Hence the stiffness matrix, $S_{c,d}$, has been tuned to $S_{c,d}$ = $diag\{20, 20, 20, 50, 50, 50\}$, while the damping matrix value is $D_{c,d}$ = $diag\{15, 15, 15, 100, 100, 100\}$.    
 %============================================
 \begin{figure}[!h]
 	\centering
 	\includegraphics[width=0.6\columnwidth]{wind_angle}
 	\caption{Profile of the wind angle}
 	\label{fig:wind_angle}
 \end{figure}
%============================================
 %============================================
 \begin{figure}[!h]
 	\centering
 	\includegraphics[width=0.6\columnwidth]{wind_speed}
 	\caption{Profile of the wind speed}
 	\label{fig:wind_speed}
 \end{figure}
 %============================================
\begin{table}[!h]
	\caption{FTRLS-DOB simulation parameters}
	\label{tab:ftrls_DOb_par}
	\begin{center}
		\setlength{\tabcolsep}{0.01pt}
		\begin{tabular}{|c|c|}
			\hline
			Parameter & Value\\ 
			\hline
         	$A_{e_1}$ & $0.16$ \\
			\hline
			$S_{c,d}$ & $diag\{20, 20, 20, 50, 50, 50\}$ \\
			\hline
			$D_{c}$ & $diag\{0, 0, 10, 0, 0, 0\}$ \\
			\hline
			$M_{c,d}$ & $2 I_6$ \\
			\hline
			$D_{c,d}$ & $diag\{15, 15, 15, 100, 100, 100\}$\\
			\hline
            $A_{e_2}$ & $0.032$ \\
			\hline
			$\eta^{min}_{h}$ & $0.8$\\
			\hline
			$\gamma_{g}$ & $5$ \\
			\hline
			$S_{c}$	& $diag\{0, 0, 20, 0, 0, 0\}$\\  
			\hline
			$z_0$& $1$ \\
			\hline
			$K_{p_\sigma}$, $K_{d_\sigma}$& $20 I_2$ \\ 
			\hline
			$K_{P,e}$ & $diag\{25, 25, 150, 200, 200, 500\}$ \\
			\hline
			$K_{D,e}$ & $diag\{15, 15, 100, 100, 500, 100\}$ \\
			\hline
		\end{tabular}
	\end{center}
\end{table}
%============================================================
\subsubsection{Estimation of the End-effector Contact Force}

Figs. \ref{fig:Fe} shows the actual end-effector contact force and its estimation. \ref{fig:Fen} illustrates the norm of the contact force estimation error. From these figures, it is possible to recognize that before instant 50 s there is no contact with the environment and the contact starts at instant 50 s. In addition, it is observed that the norm error of the end-effector generalized force in all directions have vales around zero during the non-contact period. At instant 50 s, at which the contact occurs, there is an increase in the estimation error norm. The norm of estimation error in both $x$ and $y$ directions have maximum value of $0.016$ N and $0.013$ N, respectively. While it has value of $0.03$ N in the $z$ direction, which is equivalent to 1.8 \% with respect to the actual value. In $\phi$, $\psi$ and $\theta$ directions, the norms reach value of $0.0001$ N.m. Thus, it is possible to appreciate the estimation performance of the end-effector generalized forces. Consequently, one can contend that the control objective \ref{obj:force} is achieved.

%============================================
\begin{figure}[!h]
	\centering
	\begin{tabular}{cc}
		\subfloat[$x_{e}$]{\includegraphics[width=0.4\columnwidth]{force_dob_x}}&
		\subfloat[$y_{e}$]{\includegraphics [width=0.4\columnwidth]{force_dob_y}}\\
		\subfloat[$z_{e}$]{\includegraphics [width=0.4\columnwidth]{force_dob_z}}&
		\subfloat[$\phi_{e}$]{\includegraphics [width=0.4\columnwidth]{force_dob_phe}}\\
		\subfloat[$\theta_{e}$]{\includegraphics [width=0.4\columnwidth]{force_dob_the}}&
		\subfloat[$\psi_{e}$]{\includegraphics [width=0.4\columnwidth]{force_dob_epe}}
	\end{tabular}
	\caption{FTRLS-DOb results: Actual response of the estimation of the contact force}
	\label{fig:Fe}
\end{figure}
%================================================================
\begin{figure}[!h]
	\centering
	\begin{tabular}{cc}
		\subfloat[$x_{e}$]{\includegraphics[width=0.4\columnwidth]{Fnorm_traj_force_dob_x}}&
		\subfloat[$y_{e}$]{\includegraphics [width=0.4\columnwidth]{Fnorm_traj_force_dob_y}}\\
		\subfloat[$z_{e}$]{\includegraphics [width=0.4\columnwidth]{Fnorm_traj_force_dob_z}}&
		\subfloat[$\phi_{e}$]{\includegraphics [width=0.4\columnwidth]{Fnorm_traj_force_dob_phe}}\\
		\subfloat[$\theta_{e}$]{\includegraphics [width=0.4\columnwidth]{Fnorm_traj_force_dob_the}}&
		\subfloat[$\psi_{e}$]{\includegraphics [width=0.4\columnwidth]{Fnorm_traj_force_dob_epe}}
	\end{tabular}
\caption{FTRLS-DOb results: Error norm of the estimation of the contact force}
	\label{fig:Fen}
\end{figure}
%================================================================

\subsubsection{Impedance Control}
Fig. \ref{fig:inv_kin_ftrls_results} shows the response of the system in the task space (the actual end-effector position and orientation can be found from the forward kinematics). From this figure, it is possible to recognize that the controller has good tracking of the desired trajectories of the end-effector due to the using of the tracking controller during the period of non-contact. It also possible to recognize that at the time of the contact the required impedance is applied and this produces small error in the position tracking to satisfy the impedance requirements. 
%======================ot===========
\begin{figure}[!h]
	\centering
	\begin{tabular}{cc}
		\subfloat[$x_{e}$]{\includegraphics[width=0.4\columnwidth]{xe_traj_force_dob}}&
		\subfloat[$y_{e}$]{\includegraphics [width=0.4\columnwidth]{ye_traj_force_dob}}\\
		\subfloat[$z_{e}$]{\includegraphics [width=0.4\columnwidth]{ze_traj_force_dob}}&
		\subfloat[$\phi_{e}$]{\includegraphics [width=0.4\columnwidth]{phe_traj_force_dob}}\\
		\subfloat[$\theta_{e}$]{\includegraphics [width=0.4\columnwidth]{the_traj_force_dob}}&
		\subfloat[$\psi_{e}$]{\includegraphics [width=0.4\columnwidth]{epe_traj_force_dob}}
	\end{tabular}
	\caption{FTRLS-DOb results: The actual response of the end-effector pose: a) $x_{e}$, b) $y_{e}$, c) $z_{e}$, d) $\phi_{e}$, e) $\theta_{e}$, and f) $\psi_{e}$}
	\label{fig:inv_kin_ftrls_results}
\end{figure}
%==============================================
%==============================================
Fig. \ref{fig:DOb_3d} shows the motion of the end-effector in the 3D dimension (The markers represent the orientation). These results show that the proposed impedance motion control scheme provides a robust performance to track the desired end-effector trajectories as well as to achieve the desired impedance effect on the environment taken into consideration the external disturbances and noises. As a result, one can claim that the control objectives \ref{obj:stab}, \ref{obj:track}, and \ref{obj:impd} are achieved. 
%==================================================
\begin{figure}[!h]
	\centering
	\includegraphics[width=0.7\columnwidth]{3D_traj_force_dob}
	\caption{FTRLS-DOb results: 3D trajectory of the end-effector pose (The marker represents the end-effector orientation; Green, Blue, and Red for x-,y-, and z-axis, respectively)}
	\label{fig:DOb_3d}
\end{figure}
%=================================
Finally, Fig. \ref{fig:inv_kin_ftrls_joint} shows the actual trajectories of the system in the quadrotor/joint space from which it is noted that the generated trajectories in the quadrotor/joint space are in the allowable limits of the manipulator joints.
%=================================
\begin{figure}[!h]
	\centering
	\begin{tabular}{cc}
		\subfloat[$x_{e}$]{\includegraphics[width=0.4\columnwidth]{x_traj_force_dob}}&
		\subfloat[$y_{e}$]{\includegraphics [width=0.4\columnwidth]{y_traj_force_dob}}\\
		\subfloat[$z_{e}$]{\includegraphics [width=0.4\columnwidth]{z_traj_force_dob}}&
		\subfloat[$\psi$]{\includegraphics [width=0.4\columnwidth]{ep_traj_force_dob}}\\
		\subfloat[$\theta_{1}$]{\includegraphics [width=0.4\columnwidth]{th1_traj_force_dob}}&
		\subfloat[$\theta_{2}$]{\includegraphics [width=0.4\columnwidth]{th2_traj_force_dob}}
	\end{tabular}
	\caption{FTRLS-DOb results: The actual trajectories of the variables in the quadrotor/joint space}
	\label{fig:inv_kin_ftrls_joint}
\end{figure}

==> 6_Conclusions/Conclusions.tex <==
% this file is called up by thesis.tex
% content in this file will be fed into the main document

\chapter{CONCLUSIONS} % top level followed by section, subsection
\label{ch:Conclusions}

% ----------------------- paths to graphics ------------------------

% change according to folder and file names
\ifpdf
    \graphicspath{{7_Conclusions/figures/PNG/}{7_Conclusions/figures/PDF/}{7_Conclusions/figures/}}
\else
    \graphicspath{{7_Conclusions/figures/EPS/}{7_Conclusions/figures/}}
\fi


% ----------------------- contents from here ------------------------
\section{Conclusions}

This thesis presents the development of control design and practical implementation of a new non-redundant quadrotor manipulation system that has superior features over the currently developed systems and has vital applications. The following conclusions are obtained: 

\begin{enumerate}
	\item Successful experimental verification is done for the design of a new quadrotor manipulation system that its 2-DOF manipulator has unique topology to enable the end-effector to track arbitrary 6-DOF trajectory. This system provide solutions to limitations found in the currently developed aerial manipulation systems by having maximum mobility with minimum weight.
	  

	\item The system parameters are identified to be utilized in both controller implementation and simulation of the developed dynamic model of the system.
	
	\item A measurement and estimation scheme is proposed and implemented to get the six states representing the position and orientation of the system by using the onboard sensors. In contrast to previous works, this scheme enables utilizing the system within arbitrary place indoors and provides potential to work outdoors as well. This makes the system capable to do real practical applications.

	\item The proposed system feasibility and efficiency are proved in both simulation and experiment with a scenario consisting of taking off with an object, moving, and releasing it at a desired position. Both simulation and experimental results demonstrate a satisfactory performance. 


  \item A novel inverse kinematics analysis is carried out  to transform the  task space trajectory to  quadrotor/joint space trajectory and hence enables controlling the system in the  quadrotor/joint space. Such analysis has not been done before either for redundant or non-redundant aerial manipulator. 
  
  \item An algorithm is developed to get approximate solution to the complex differential algebraic equations resulted from the inverse kinematics analysis that incorporate the high order nonholonomic constraints of the system.  
  
   \item Numerical results validate the high accuracy of the inverse kinematics solution.
  
  \item The success of the inverse kinematics proves the ability of the system to track arbitrary 6-DOF task space trajectories that lay within the capability of the system's actuators.
  
\item A quite realistic simulation setup is built to test the developed control systems.

\item Numerical results show robust performance and satisfactory tracking of a desired 6-DOF task space trajectory using the developed DOb-based controller. A modification of the DOb-based controller is carried out to use the direct measurements from the onboard sensors in order to reduce the disturbance estimation error.

\item Optimum performance while keeping the control signal within the allowable limits is achieved by developing a robust optimal control based on the DOb and MPC approaches. Numerical results show that the control efforts are reduced and thus the mission time is increased. 
 
\item A robust sensorless force estimation and impedance control scheme is developed based on the FTRLS and DOb techniques, which takes into consideration all the system dynamics with no need for the environment contact indication. The efficiency of the proposed control systems is validated via numerical results. 



\end{enumerate}


\section{Future Plans}

\noindent Following are some of the problems for future research work:

\begin{itemize}
	
\item Increasing the accuracy of the measurement of the position in $z$-axis. This can be done by replacing the sonar with a downward laser beams.

\item Repeat the experiment with more sophisticated tasks indoors and in the field outdoors.

\item In addition to the laser ranger, vision based localization and navigation scheme can be built to improve the motion accuracy both indoors and specially outdoors.

\item Robust state estimation to increase the accuracy of the state estimation.


\item Experimental implementation of the inverse kinematics, PD-DOb, MPC-DOb, and FTRLS-DOb algorithms to verify their efficiency in real time.

\item Autonomous motion for picking and placing an object or implementing specific task.  

\end{itemize} 

% ---------------------------------------------------------------------------
% ----------------------- end of thesis sub-document ------------------------
% --------------------------------------------------------------------------- 
